Counterfactual Causality for Reachability and Safety based on Distance Functions

Investigations of causality in operational systems aim at providing human-understandable explanations of why a system behaves as it does. There is, in particular, a demand to explain what went wrong on a given counterexample execution that shows that a system does not satisfy a given specification. To this end, this paper investigates a notion of counterfactual causality in transition systems based on Stalnaker's and Lewis' semantics of counterfactuals in terms of most similar possible worlds and introduces a novel corresponding notion of counterfactual causality in two-player games. Using distance functions between paths in transition systems, this notion defines whether reaching a certain set of states is a cause for the violation of a reachability or safety property. Similarly, using distance functions between memoryless strategies in reachability and safety games, it is defined whether reaching a set of states is a cause for the fact that a given strategy for the player under investigation is losing. The contribution of the paper is two-fold: In transition systems, it is shown that counterfactual causality can be checked in polynomial time for three prominent distance functions between paths. In two-player games, the introduced notion of counterfactual causality is shown to be checkable in polynomial time for two natural distance functions between memoryless strategies. Further, a notion of explanation that can be extracted from a counterfactual cause and that pinpoints changes to be made to the given strategy in order to transform it into a winning strategy is defined. For the two distance functions under consideration, the problem to decide whether such an explanation imposes only minimal necessary changes to the given strategy with respect to the used distance function turns out to be coNP-complete and not to be solvable in polynomial time if P is not equal to NP, respectively.

==> sections/app_approx-dHH.tex <==
\subsection{Approximative algorithm for Hausfdorff-Hamming distance}
\label{app:approx}

\todo[inline]{To review}
Now, we give a constructive algorithm to compute a winning strategy that 
minimise the Hausdorff-Hamming distance with the non-winning strategy. This 
algorithm is not in polynomial time, a priori, since it uses a solution of an 
instance of the feedback vertex set problem.

\begin{proposition}
	\label{prop:finding-trans_algo}
	Let \game be a reachable game, and \loosestrategy be a non-winning strategy. 
	We can build \winstrategy be a winning strategy such that \winstrategy 
	minimise the Hausdorff-Hamming distance with \loosestrategy, i.e. 
	$\winstrategy = \min_{\strategy-\text{winning}} \dHH(\loosestrategy, 
	\strategy)$.
\end{proposition}

The proof of this proposition consists by definition a winning strategy for 
\ReachPl player that minimise $\dstrat{\winstrategy}(\loosestrategy)$. Then, 
after changing a little it to obtain a winning strategy that minimise 
$\dstrat{\loosestrategy}(\winstrategy)$ without increase 
$\dstrat{\winstrategy}(\loosestrategy)$, we obtain the \winstrategy of 
the proposition. More precisely, this algorithm is split into three steps where 
the last one corresponding to the feedback vertex set problem:  
\begin{enumerate}
	\item we define by a reduction to the shortest-path game, 
	a winning strategy \winstrategy in \game such that \winstrategy minimises 
	(over winning strategies) $\dstrat{\winstrategy}(\loosestrategy)$ distance 
	(see Lemma~\ref{lem:DHH-strat_find}); 
	\item we synchronise \winstrategy and \loosestrategy for 
	vertices that are unreachable under \winstrategy without change the distance 
	$\dstrat{\winstrategy}(\loosestrategy)$ (see 
	Lemma~\ref{lem:DHH-strat_transformation1}); 
	\item\label{item:algo_FVS} we synchronise \winstrategy and \loosestrategy for 
	a maximal number of vertices into SCC defined under \loosestrategy without 
	change the distance $\dstrat{\winstrategy}(\loosestrategy)$ (see 
	Lemma~\ref{lem:DHH-strat_transformation2}).
\end{enumerate}
In the following, we will discuss about each step.


\begin{lemma}
	\label{lem:DHH-strat_transformation3}
	$\winstrategy^1$ is an optimal MD-strategy in \game and 
	$\dstrat{\loosestrategy}(\winstrategy) \geq 
	\dstrat{\loosestrategy}(\winstrategy^1)$.
\end{lemma}
\begin{proof}
	We start by proving that $\winstrategy^1$ is an optimal MD-strategy in 
	\game. To do that, we will prove that all $\winstrategy^1$-plays are 
	also a \winstrategy-play. We reason by contraction and we suppose that 
	\winplay is a $\winstrategy^1$-play but not a \winstrategy-play. In 
	particular, there exists a vertex $\loc \in \LocsReach$ such that 
	$\winstrategy^1(\loc) \neq \winstrategy(\loc)$ (and without lost of 
	generality, we take the first one). By definition of $\winstrategy^1$, we 
	know that \loc is not in the connected component that contains 
	$\locinit$ (otherwise, both decision are equal). However, the prefix of 
	\winplay until \loc is also a \winstrategy-play (like we have chosen 
	\loc like the first vertex along \winplay such that both strategies are 
	distinct). In particular, \loc is in the connect component of $\locinit$ 
	(as there exists a path between $\locinit$ and \loc in the non-directed 
	graph underlying by $\game^{\winstrategy}$). We obtain a contradiction, and 
	like all $\winstrategy^1$-plays are also a \winstrategy-play, we 
	deduce that $\sCost(\winstrategy^1) \leq \sCost(\winstrategy)$. We conclude 
	by optimality of \winstrategy.
	
	Now, we prove that $\dstrat{\loosestrategy}(\winstrategy) \geq 
	\dstrat{\loosestrategy}(\winstrategy^1)$. In particular, we want to prove 
	that for all \looseplay be a \loosestrategy-play, we have 
	$\dist(\looseplay, \winstrategy^1) \leq \dist(\looseplay, \winstrategy)$. We
	reason by induction on the length of \looseplay. If $\looseplay = \locinit$ 
	then $\dist(\looseplay, \winstrategy^1) = 0 = 
	\dist(\looseplay, \winstrategy)$, since there are no choices. 
	
	Now, we suppose that $\looseplay = \looseplay' \loc$ where we denote the last 
	vertex of \looseplay by $\loc'$. If $\loc' \in \LocsSafe$, then the 
	last choice of \looseplay does not occur for the computation of $\dist$, 
	and we have 
	\begin{displaymath}
	\dist(\looseplay, \winstrategy^1) = \dist(\looseplay', \winstrategy^1) 
	\qquad \text{and} \qquad
	\dist(\looseplay, \winstrategy) = \dist(\looseplay', \winstrategy). 
	\end{displaymath} 
	We conclude that $\dist(\looseplay, \winstrategy^1) \leq 
	\dist(\looseplay, \winstrategy)$ by hypothesis of induction applying to 
	$\looseplay'$. If, $\loc' \in \LocsReach$ and $\winstrategy(\loc') = 
	\loosestrategy(\loc')$, then by $\winstrategy^1(\loc') = 
	\loosestrategy(\loc')$ (by it definition), and we have 
	\begin{displaymath}
	\dist(\looseplay, \winstrategy^1) = \dist(\looseplay', \winstrategy^1) 
	\qquad \text{and} \qquad
	\dist(\looseplay, \winstrategy) = \dist(\looseplay', \winstrategy).
	\end{displaymath} 
	We conclude that $\dist(\looseplay, \winstrategy^1) \leq 
	\dist(\looseplay, \winstrategy)$ by hypothesis of induction applying to 
	$\looseplay'$. Otherwise, $\loc' \in \LocsReach$ and $\winstrategy(\loc') 
	\neq \loosestrategy(\loc')$. In this case we have 
	\begin{displaymath}
	\dist(\looseplay, \winstrategy^1) = 
	\begin{cases}
	\dist(\looseplay', \winstrategy^1) + 1 & \text{if $\loc'$ belongs to the 
		connected component of $\locinit$} \\
	\dist(\looseplay', \winstrategy^1) & \text{otherwise} \\
	\end{cases} 
	\end{displaymath} 
	Moreover, $\dist(\looseplay, \winstrategy) = \dist(\looseplay', \winstrategy) 
	+ 1$. We conclude that $\dist(\looseplay, \winstrategy^1) \leq 
	\dist(\looseplay, \winstrategy)$ by hypothesis of induction applying to 
	$\looseplay'$. \qed
\end{proof}

\paragraph{Step~\ref{item:algo_FVS}: the feedback vertex set problem reduction}
To minimise the distance $\dstrat{\loosestrategy}(\winstrategy)$ in 
\game, \winstrategy needs to follow \loosestrategy as long as possible: in 
the best case, we want to follow \loosestrategy in all vertices of the cycle 
except the last one. In particular, we want to compute the minimal feedback 
vertex set. 

Intuitively, we want use this problem to compute the set of vertex where 
\winstrategy and \loosestrategy must be distinct. However, we can not 
directly apply this problem on the graph underlying by \game or 
$\game^{\loosestrategy}$, we need a transformation of this graph: we want to 
remove the vertex of \SafePl as we can not make any constraints on its 
choices, and vertex of \ReachPl where \winstrategy and \loosestrategy are 
already the same choice since we need to grantee that the chosen vertices by 
the problem has an outgoing transition by \winstrategy.

More formally, let $\game^{\winstrategy, \loosestrategy} = (\Locs, \Trans)$ be a 
RG such that we only keep the decision given by \winstrategy and 
\loosestrategy in all vertices of \ReachPl. For all SCC $\C$ in 
$\game^{\winstrategy, \loosestrategy}$, we define $G_{\C}' = (\Locs'', \Trans'')$ be the graph underlying $\C$ where we remove all vertices of \ReachPl such 
that the out-going degree, denoted by $out$, is equal to $1$. 
Formally, we define $G_{\C}'$ such that 
\begin{itemize}
	\item $\Locs'' = \{\loc ~|~ \loc \in \LocsSafe \text{ or } \loc \in \ReachPl 
	\text{ s.t. } out(\loc) = 1\}$;
	\item \begin{align*}
	\Trans'' &= \{(\loc, \loc') ~|~ (\loc, \loc') \in \Trans\} \\
	&\cup \{(\loc, \loc') ~|~ \exists (\loc, \loc''), (\loc'', \loc) \in \Trans 
	\text{ s.t. } \loc'\in \LocsReach \text{ and } out(\loc') = 1 \}
	\end{align*}
\end{itemize}
To conclude, this reduction to the feedback vertex set problem, we need to remove 
all vertices of \SafePl in $G_{\C}'$. Formally, we define 
$G_{\C} = (\Locs', \Trans')$ such that 
\begin{itemize}
	\item $\Locs' = \{\loc ~|~ \loc \in \LocsReach'\}$;
	\item $\Trans' = \{(\loc, \loc') ~|~ (\loc, \loc') \in \Trans''\} \cup 
	\{(\loc, \loc') ~|~ \exists (\loc, \loc''), (\loc'', \loc) \in \Trans'' 
	\text{ s.t. } \loc'\in \LocsSafe \}$.
\end{itemize}

\begin{figure}[tbp]
	\centering
	\begin{tikzpicture}[xscale=.7,every node/.style={font=\footnotesize}, 
	every label/.style={font=\scriptsize}]
	\node[PlayerReach] at (0, 0) (v0) {$\loc_0$};
	\node[PlayerReach] at (2, 1.5) (v1) {$\loc_1$};
	\node[PlayerSafe] at (2,-1.5) (v2) {$\loc_2$};
	\node[PlayerReach] at (4, 0) (v3) {$\loc_3$};
	\node[target] at (-1.5, 0) (t1) {};
	\node[target] at (.5, 1.5) (t2) {};
	
	% Connect the states with arrows
	\draw[->] 
	(v0) edge (v1)
	(v0) edge (t1)
	(v1) edge (t2)
	(v1) edge (v3)
	(v2) edge (v1)
	(v2) edge (v0)
	(v3) edge (v2);
	
	\begin{scope}[xshift=7cm]
	\node[PlayerReach] at (0, 0) (v0) {$\loc_0$};
	\node[PlayerReach] at (2, 1.5) (v1) {$\loc_1$};
	\node[PlayerSafe] at (2,-1.5) (v2) {$\loc_2$};
	
	% Connect the states with arrows
	\draw[->] 
	(v0) edge (v1)
	(v1) edge[bend left=10] (v2)
	(v2) edge[bend left=10] (v1)
	(v2) edge (v0);
	\end{scope}
	
	\begin{scope}[xshift=11cm]
	\node[PlayerReach] at (2, 1.5) (v1) {$\loc_1$};
	\node[PlayerReach] at (2,-1.5) (v2) {$\loc_0$};
	
	% Connect the states with arrows
	\draw[->] 
	(v1) edge[loop right] (v1)
	(v1) edge[bend left=10] (v2)
	(v2) edge[bend left=10] (v1);
	\end{scope}
	\end{tikzpicture}
	\caption{On the left, we have a SCC $\C$ of a game under \winstrategy and 
		\loosestrategy. On the middle, we have the graph $G_{\C}'$ be the first 
		transformation of $\C$. On the right be have $G_{\C}$ be the graph obtained 
		for the feedback vertex set problem from $\C$.}
	\label{fig:ex_red-feedback}
\end{figure}

\begin{example}
	In Figure~\ref{fig:ex_red-feedback}, we give the steps of the reduction of 
	our problem to feedback vertex set problem for one SCC. On the left, we 
	consider a SCC $\C$ of a game under \winstrategy and \loosestrategy. On 
	the middle, we have the graph $G_{\C}'$ be the first transformation of $\C$. 
	On the right be have $G_{\C}$ be the graph obtained 
	for the feedback vertex set problem from $\C$.
	\markend
\end{example}


For all SCC $\C$ of $\game^{\winstrategy, \loosestrategy}$, we let $S_{\C} 
\subseteq \LocsReach$ be the set of vertices computed by the feedback vertex 
set problem on $G_{\C}$. So, from $\winstrategy^1$, we fix, for all vertices $
\loc \in \LocsReach$, 
\begin{displaymath}
\winstrategy^2(\loc) = 
\begin{cases}
\winstrategy^1(\loc) & \text{if $\loc \notin \cup_{\C} S_C$} \\
\loosestrategy(\loc) & \text{otherwise}
\end{cases}
\end{displaymath}
To conclude this step, we need to prove that $\winstrategy^2$ remains optimal in 
\game and minimizes the distance $\dstrat{\loosestrategy}(\winstrategy)$ in 
\game. In particular, $\winstrategy^2$ is winning  and minimizes the distance 
$\dstrat{\winstrategy}(\loosestrategy)$ in \game (by 
Lemma~\ref{lem:DHH-strat_find}).


\begin{lemma}
	\label{lem:DHH-strat_transformation2}
	$\winstrategy^2$ is an optimal MD-strategy in \game and minimizes the 
	distance $\dstrat{\loosestrategy}(\winstrategy)$ in \game.
\end{lemma}
\begin{proof}
	We start by proving that $\winstrategy^2$ is an optimal MD-strategy in 
	\game. We remark that all vertices in the same SCC under 
	$\winstrategy^2$ that follow \winstrategy are the same maximal cost (otherwise, \winstrategy is not an optimal strategy).  
	Now, let \winplay be a $\winstrategy^2$-play but not a 
	$\winstrategy^1$-play. In particular, there exists $\loc \in \LocsReach$ be 
	in a SCC of $\game^{\winstrategy, \loosestrategy}$ $\C$ such that 
	$\winstrategy^1(\loc) \neq \winstrategy^2(\loc)$. Let the first vertex 
	that satisfying this condition. Now, we define $\winplay'$ such that 
	$\winplay'$ follows \winplay until \loc and after $\winstrategy^1$. By 
	Hypothesis on the maximal cost of vertex of $\C$, we know that the 
	maximal cost of $\loc'$ the last vertex of $\C$. In particular, like 
	pass in $\C$ cost $0$ both plays has the same weight.
	
	Now, we prove that $\winstrategy^2$ minimise 
	$\dstrat{\loosestrategy}(\winstrategy)$, i.e. 
	$\dstrat{\loosestrategy}(\winstrategy^2) = 
	\min_{\winstrategy \text{-winning}} \dstrat{\loosestrategy}(\winstrategy)$. 
	We reason by contradiction, and we suppose that there exists a winning 
	strategy \strategy such that $\dstrat{\loosestrategy}(\strategy) < 
	\dstrat{\loosestrategy}(\winstrategy)$. Let $\C$ be an SCC in 
	$\game^{\winstrategy, \loosestrategy}$ and let \looseplay be a 
	\loosestrategy-play that reaches all vertex of $\C$ and stay inside for 
	ever. Since by hypothesis $\dstrat{\loosestrategy}(\strategy) < 
	\dstrat{\loosestrategy}(\winstrategy)$, we know that 
	$\dist(\looseplay, \strategy) < \dist(\looseplay, \winstrategy)$. In 
	particular, there exists $\loc \in \C$ such that $\winstrategy(\loc) \neq 
	\loosestrategy(\loc)$ but $\strategy(\loc) = \loosestrategy(\loc)$. We 
	obtain a contradiction with the minimality of the set. 
	\qed	
\end{proof}


\noindent Questions: Can we obtain a polynomial time algorithm by remove the 
condition over the memory in the winning strategy? unfolding, switching, ...

==> sections/app_finding-dcause.tex <==
\section{Proof of Theorem~\ref{thm:finding-complete}}
\label{app:finding-dcause}
\todo[inline]{To review}

In this appendix, we makes the detailed proof of Theorem~\ref{thm:finding-complete}.

\findingComplete*

As explain in the main paper, for both distances, the proof is given by a reduction
to the problem of finding a $k,d$-closed winning MD-strategy with a minimal distance 
to \loosestrategy that is NP-hard by Theorem~\ref{thm:strat_finding-NP-c}. In 
particular, from a winning MD-strategy \winstrategy for \ReachPl, we define a 
$d$-strat-cause: a \emph{quasi-strat-cause given by \winstrategy} is given by the 
set of vertices: 
\begin{equation}
\label{eq:cause-from-strat}
C^{\winstrategy} = \{\loc ~|~ \loosestrategy(\loc) \neq \winstrategy(\loc) \}
\end{equation} 
In particular, by definition of $C^{\winstrategy}$, \winstrategy is a 
$C^{\winstrategy}$-distinct \loosestrategy-strategy (since it is winning). 
Thus, we deduce the following lemma, i.e. $C^{\winstrategy}$ is well a 
quasi-strat-cause.

\begin{lemma}
	\label{lem:Ctau_quasi-cause}
	Let \winstrategy be a winning strategy for \ReachPl in a reachability game \game 
	under a \loosestrategy be a non-winning strategy for \ReachPl. Then, 
	$C^{\winstrategy}$ (defined by~\eqref{eq:cause-from-strat}) is a 
	quasi-strat-cause. 
\end{lemma}

To conclude the proof of Theorem~\ref{thm:finding-complete}, we exhibit the 
reduction to the finding $k$-closed winning strategy problem. Formally, let \game 
be a reachability game where \ReachPl wins, \loosestrategy 
be a non-winning MD-strategy for \ReachPl and $k \in \N$ be a given thresholds an 
instantiation of finding a $k$-closed winning strategy problem. We recall that, by 
Theorem~\ref{thm:strat_finding-NP-c}, this problem is NP-hard for Hamming 
strategy distance and \dHH. Moreover, we remark that \game and \loosestrategy are 
also an instantiation of the finding a $k,d$-strat-cause for Hamming strategy 
distance or \dHH problem. In particular, to conclude the proof, we prove the 
following lemma.

\begin{lemma}
	The two following properties are equivalent:
	\begin{enumerate}
		\item there exists \winstrategy be a winning MD-strategy for \ReachPl such 
		that $d(\winstrategy, \loosestrategy) \leq k$;
		\item there exists $C$ be a $k,d$-strat-cause.
	\end{enumerate}
\end{lemma}
\begin{proof}
	We begin by supposing that $C$ be a $k,d$-strat-cause. In particular, by definition 
	of a such cause, there exists \winstrategy be a $C$-distinct \loosestrategy-strategy, 
	i.e. a winning MD-strategy for \ReachPl, such that 
	$d(\loosestrategy, \winstrategy) \leq k$.
	
	Conversely, we suppose that there exists \winstrategy be a winning MD-strategy for 
	\ReachPl such that $d(\winstrategy, \loosestrategy) \leq k$ and we define 
	$C^{\winstrategy}$ with~\eqref{eq:cause-from-strat}. So, by 
	Lemma~\ref{lem:Ctau_quasi-cause}, $C^{\winstrategy}$ is a quasi-strat-cause such 
	that \winstrategy is a $C^{\winstrategy}$-distinct \loosestrategy-strategy. 
	We conclude, by hypothesis on $d(\winstrategy, \loosestrategy)$.
	\qed
\end{proof}










==> sections/app_old_sections.tex <==
\section{Old Material \textcolor{red}{to be removed}}


\subsection{Finding good causes in transition systems}




\subsubsection{Minimal number of states}
\todo[inline]{This subsection  can be removed if we cannot fix it.}

\paragraph{Prefix metric.}

\begin{theorem}
Given a transition system $\cT=(S,\to,\sinit)$, a set of terminal states $E$, and an execution $\pi\vDash \lozenge E$, a cardinality-minimal $\dpref$-counterfactual cause $C$ for $E$ can be computed in polynomial time.
\end{theorem}

\begin{proof}[Proof sketch]
We add self-loops to all terminal states of $\cT$ and still refer to the edges by $\to$.

From each state $s_i$ of $\pi$ (as a new initial state), we try to find a \emph{necessary} cause $C$ for $E$ with minimal number of states such that $\exists \Box \neg C$  holds. 

We use the linear program to find a minimal cut. We add constraints that ensure that there is still a ``flow'' from $s_i$ avoiding the cut and constraints ensuring that from $s_{i+1}$ there is no flow avoiding the cut.




Variables:
\begin{itemize}
\item 
one variable $z_v$ per state $v\in S$ (will be used to mark states reachable from $s_i$ before the cause),
\item 
one variable $y_v$ per state $v\in S$ (will be used to mark states reachable from $s_{i+1}$ before the cause),
\item 
one variable $c_v$ per state $v\in S$ (will be used to mark states in the cause),
\item 
one variable $p_v$ per state $v\in S$ (will be used to check that there are no cycles within the states marked by the $y$-variables),
\item 
one variable $d_{uv}$ per edge $(u,v)\in \to$ (as in the min-cut-LP),
\item
one variable $f_{uv}$ per edge $(u,v)\in \to$ (used to check that there is still a path (or ``flow'') from $s_i$ not reaching the cause).
\end{itemize}

Goal:
\[
\text{Minimize } \sum_{v\in S} c_v
\]

subject to
\begin{align*}
z_{s_i}			&=1,			&\\
z_e				&=0, 		&\text{for all }e\in E, \\
d_{uv}-z_u+z_v		&\geq 0   		&\text{for all }(u,v)\in \to , \\
d_{uv}			&\geq 0   		&\text{for all }(u,v)\in \to , \\
c_v				&\geq d_{uv}	&\text{for all }(u,v)\in \to , \\
				&&{  \text{(min-cut-LP)}} \\
				&			& \\
f_{uv}			&\geq 0   		&\text{for all }(u,v)\in \to , \\
f_{uv}			&\leq z_v   		&\text{for all }(u,v)\in \to , \\
f_{uv}			&\leq z_u   		&\text{for all }(u,v)\in \to , \\
\sum_{(v,u)\in \to} f_{vu} &= \sum_{(u,w)\in \to} f_{uw}  & \text{for all } u\in S, \\
\sum_{(v,u)\in \to} f_{vu} &\geq 1, 	&\\
							&&{  \text{(existence of a cycle before the cause)}}\\
				&			& \\
y_{s_{i+1}}		&=z_{s_{i+1}},	& \\
y_e				&=0, 		&\text{for all }e\in E, \\
d_{uv}-y_u+y_v		&\geq 0   		&\text{for all }(u,v)\in \to , \\
p_u				&\geq p_v +y_u+y_v-1   	&\text{for all $u,v$ reachable from $s_{i+1}$ with $(u,v)\in \to$}.\\
							&&{  \text{(no path from $s_{i+1}$ not reaching the cause)}}
\end{align*}



Any cardinality minimal cause $C$ with $k$ states induces a solution to the linear program for some state $s_i$ with $\sum_{v\in S} c_v=k$.
Vice versa, for any solution to the linear program, we can assume that it lies on a vertex of the feasible region. This should imply that all relevant variables are $0$ or $1$. The set
of nodes $v$ with $c_v=1$ forms a cause, the variables $f_{uv}$ witness that a cycle is still reachable before the cause is reached.
\textcolor{red}{needs to be checked}
\qed
\end{proof}
\todo{For the min-cut LP, it can be shown that the LP has an integral solution by showing that the matrix in the linear constraints is totally unimodular. I think, this is not the case here anymore.}




\paragraph{Hamming distance.}

unclear.


\paragraph{Levenshtein distance.}

unclear.







\subsection{Hausdorff distance $\dhamm^H$ based on Hamming distance $\dhamm$.}
\todo[inline]{Check and complete this section. Does the result hold? }
\todo[inline]{Jakob: Do the NP-hardness results for finding winning strategies with bounded distance to a given strategy below transfer to some decision problems for this counterfactual definition, e.g., checking whether $C$ is a Hamming-distance-counterfactual cause? 
What about finding small causes? Here the potential hardness seems be of a different nature in case checking whether a candidate is a cause is in P.}

Now, we study counterfactual causes defined with the Hausdorff distance based on the 
Hamming distance. Intuitively, letting \winstrategy and \loosestrategy 
be two memoryless strategies, this distance between \winstrategy and \loosestrategy 
computes the minimal numbers of new vertices needed to transform a 
\winstrategy-play into a \loosestrategy-play, and vice versa. Then, this distance
take the maximal between the two numbers.


As in the transition systems setting, the Hamming distance is not defined on plays of 
different length. So, in this section, we suppose that the considered reachability 
game $\game =  (\Locs, \locinit, \Trans)$ is acyclic and all its plays have the same 
length. More formally, we suppose that we can decompose \Locs such that 
$\Locs = \cup_{i=0}^n \Locs_i$ with $\Locs_0 = \{\locinit\}$, 
$\Locs_n = \LocsT \cup \neg\LocsT$  where $\neg\LocsT = 
\{\loc \mid \loc \notin \LocsT \text{ and } \Trans(\loc) = \emptyset\}$, and for 
all $i \in (0, n)$, $\Locs_i$ contains vertices at distance $i$ of \locinit.
Given a set of locations $C$ as potential cause and a strategy $\sigma$ for $\SafePl$, we want to check if $C$ is a 
$\dhamm^H$-counterfactual cause for the fact that $\sigma$ loses in $\game$. 

\begin{theorem}
	\label{thm:check-counterfactual-game}
	Let \game be an acyclic reachability game where all plays have the same 
	length and \SafePl wins. Let \loosestrategy be a non-winning strategy 
	for \SafePl, and $C \subseteq \Locs$ be a candidate counterfactual-cause. 
	Then, we can test in polynomial time if $C$ is a $\dhamm^H$-counterfactual 
	cause.
\end{theorem} 

As explained in the case of the Hausdorff distance based in the prefix distance, 
the two first conditions of Definition~\ref{def:game_conterfactual-cause} can be 
check in polynomial time by considering an attractor for $C$. Thus, we only need to test 
the last condition by adapting the proof of Theorem~\ref{thm:checking_dhamm} that 
checks  $\dhamm$-counterfactual causality in transitions systems: we want to make a 
comparison between a "shortest-path" (defined according to the non-winning strategy) 
that avoids $C$ and reaches a non-effect leaf, and a "shortest-path" that avoids $C$ 
and that reaches the effect.

Formally, from $\game = (\Locs, \locinit, \Trans)$ such that \Locs is split by 
$\Locs = \cup_{i=0}^n \Locs_n$ and a non winning strategy \loosestrategy, we define 
a shortest-path game $\widetilde{\game}_\loosestrategy = 
(\widetilde{\Locs}, \locinit, \Trans, \weight)$ such that 
$\widetilde{\Locs} = \LocsMin \uplus \LocsMax \uplus \LocsT \uplus \LocsNegT$ where 
$\LocsMin = \LocsSafe$, $\LocsMax = \LocsReach$ and $\Locs_T = \LocsNegT$. The 
weight function is given for all edges $(\loc, \loc') \in \Trans$ and all 
vertices $\loc \in \Locs$ by
\begin{displaymath}
	\weight(\loc, \loc') = 
	\begin{cases}
	1 & \text{if $\loc \notin \game^{\loosestrategy}$} \\
	0 & \text{otherwise}
	\end{cases} 
	\qquad \text{and} \qquad
	\weight(\loc) = 
	\begin{cases}
	1 & \text{if $\loc \in \Locs_T \setminus \Locs^{\loosestrategy}$} \\
	0 &\text{if $\loc \in \Locs_T \cap \Locs^{\loosestrategy}$} \\
	+\infty & \text{otherwise}
	\end{cases} 
\end{displaymath}
\todo[inline]{Jakob: I do not see how this weight function relates to the paths that actually exist in $\game^\sigma$.
Also, the Hamming distance was defined on labels. I think, however, we could just use it on states here...}
\todo[inline]{Julie : For instance, we do not gives some labels in games.}
\figurename{\ref{fig:game_counterfactual-cause}} illustrates this transformation.
Intuitively, the cost of \winstrategy computes the minimum number of vertices that 
are not in $\game^{\loosestrategy}$ need to avoid the effect, i.e. reach $\Locs_T$.
Then, this shortest-path game encodes the Hausdorff-Hamming distance between 
a given strategy \winstrategy and \loosestrategy by the cost of \winstrategy. 
In particular, the cost of \game computes the minimal Hausdorff-Hamming distance 
between an optimal strategy and \loosestrategy. 

\begin{remark}
	As explain in Section~\ref{sec:prelim}, we can define an equivalent shortest-path 
	game (without weight on vertices) by adding a new level $V_{n+1}$ that will be 
	contains a target leaf and a non-target leaf. Now, all vertices in $\LocsNegT$ 
	are linked with the target (and a weight $1$ if there are not in 
	$\game^{\loosestrategy}$), and all vertices of $\LocsT$ are linked with the 
	non-target leaf. 
	\markend
\end{remark}

\begin{figure}[tbp] 
	\centering
	\begin{tikzpicture}[xscale=.7,every node/.style={font=\footnotesize}, 
	every label/.style={font=\scriptsize}]
	\node[PlayerSafemin] at (0,0) (s0) {};
	\node[PlayerSafemin] at (2,-1) (s1) {};
	\node[PlayerReachmin] at (2, 1) (s2) {};
	\node[PlayerReachmin] at (4,-1) (s3) {};
	\node[PlayerSafemin] at (4, 0.5) (s4) {};
	\node[PlayerReachmin] at (4, 1.5) (s5) {};
	\node[target] at (6,-.25) (e) {$\LocsNegT$};
	\node[target] at (6,1) (e1) {$\LocsT$};
	
	\node[strat] at (1, .5) (st1) {};
	\node[strat] at (5, .75) (st2) {};
	
	\draw[->]
	(s0) edge (s1)
	(s0) edge (s2)
	(s1) edge (s3)
	(s2) edge (s4)
	(s2) edge (s5)
	(s3) edge (e)
	(s4) edge (e)
	(s4) edge (e1)
	(s5) edge (e1)
	;
	
	\draw[DarkOrchid, ->, line width=0.5mm]
	(s0) edge (st1)
	(s4) edge (st2)
	;
	
	
	\begin{scope}[xshift=9cm]
	\node[PlayerSafemin] at (0,0) (s0) {};
	\node[PlayerSafemin] at (2,-1) (s1) {};
	\node[PlayerReachmin] at (2, 1) (s2) {};
	\node[PlayerReachmin] at (4,-1) (s3) {};
	\node[PlayerSafemin] at (4, 0.5) (s4) {};
	\node[PlayerReachmin] at (4, 1.5) (s5) {};
	\node[target] at (6,-.25) (e) {$\locNegT$};
	\node[target] at (6,1) (e1) {$\locT$};
	
	\node[strat] at (1, .5) (st1) {};
	\node[strat] at (5, .75) (st2) {};
	
	\draw[->]
	(s0) edge node[below, xshift=-.05cm] {$1$} (s1)
	(s0) edge node[above, xshift=-.05cm] {$0$} (s2)
	(s1) edge node[below] {$1$} (s3)
	(s2) edge node[below, xshift=-.05cm] {$0$} (s4)
	(s2) edge node[above, xshift=-.05cm] {$0$} (s5)
	(s3) edge node[below, xshift=.05cm] {$1$} (e)
	(s4) edge node[below, xshift=-.05cm] {$0$} (e)
	(s4) edge node[below, xshift=-.05cm] {$1$} (e1)
	(s5) edge node[above, xshift=-.05cm] {$0$} (e1)
	;
	\end{scope}
	
	\end{tikzpicture}
	\caption{On the left, a reachability game \game where all plays have the same 
		length and \SafePl wins. Vertices of \SafePl are depicted by squares, and 
		the ones of \ReachPl are by circles. In violet, we depict \loosestrategy, a 
		non-winning strategy for \SafePl. On the right, the shortest path game 
		defined from \game and \loosestrategy is depicted where vertices of \MinPl are  squares, the ones of \MaxPl are circles, and $\Locs_T = \{\locT\}$.}
	\label{fig:game_counterfactual-cause}
\end{figure}

\begin{proposition}
	\label{prop:counterfact-game_dHamm}
	Let \winstrategy be a winning strategy for \MinPl in $\widetilde{\game}$ (i.e. for 
	\SafePl in \game). Then, 
	\begin{displaymath}
	\sCost(\winstrategy) = \dhamm^H(\loosestrategy, \winstrategy).
	\end{displaymath}
	\markend
\end{proposition}

Let \winplay be a \winstrategy-play, we note that $\weight(\winplay)$ computes 
the number of vertices that are not in $\game^{\loosestrategy}$ along \winplay. 
In particular, it computes the minimal number of vertices that are not in a 
\loosestrategy-play (since all plays in $\game^{\loosestrategy}$ are 
\loosestrategy-plays).

\begin{lemma}
	\label{lem:counterfact-game_dHamm-1}
	Let \winstrategy be a winning strategy for \MinPl in $\widetilde{\game}$ (i.e. 
	all \winstrategy-plays reaches $\Locs_T$). Then, for all \winplay be a 
	\winstrategy-play, we have 
	\begin{displaymath}
	\cost(\winplay) = \inf_{\looseplay \mid \text{\loosestrategy-play}} 
	\dhamm(\winplay, \looseplay).
	\end{displaymath}
	\markend
\end{lemma}
\begin{proof}
	First, we note that \winstrategy exists since \SafePl wins in \game (by 
	hypothesis). In particular, in \game there exists \strategy be a winning 
	strategy for \SafePl and by hypothesis on \game, all \strategy-plays reaches 
	\LocsNegT, i.e. $\Locs_T$ in $\widetilde{\game}$.
	
	Now, by induction on $i$ (be the length of \winstrategy-plays reaching 
	$\Locs_T$), we prove that for all \winplay be a \winstrategy-play 
	from $\Locs_{n-i}$ in \game, we have
	\begin{enumerate}
		\item\label{item:counterfact-game_dHamm-1} 
		for all \looseplay be a \loosestrategy-play from $\Locs_{n-i}$, we have 
		$\weight(\winplay) \leq \dhamm(\looseplay, \winplay)$;
		\item\label{item:counterfact-game_dHamm-2} 
		there exists \looseplay be a \loosestrategy-play from $\Locs_{n-i}$ such 
		that $\weight(\winplay) = \dhamm(\looseplay, \winplay)$.
	\end{enumerate}
	First, we suppose that $i = 0$, and let $\winplay = \loc \in V_n$. Since, 
	\winstrategy is a winning strategy in $\widetilde{\game}$, $\loc \in \Locs_T$. 
	In case where $\loc \in \Locs^{\loosestrategy}$, by definition 
	of $\widetilde{\game}$, $\weight(\winplay) = 0$. And since for all $\loc' \in \Locs_n$,  $\dhamm(\loc, \loc') \geq 0$, \ref{item:counterfact-game_dHamm-1} 
	holds. Moreover, \loc is also a \loosestrategy-play such that 
	$\dhamm(\loc, \loc) = 0$. In particular, in this 
	case~\ref{item:counterfact-game_dHamm-2} holds. Otherwise, we suppose that 
	$\loc \notin \Locs^{\loosestrategy}$ and (by definition of $\widetilde{\game}$) 
	$\weight(\winplay) = 1$. Since $\loc \notin \Locs^{\loosestrategy}$, for all 
	$\loc' \in \Locs_n \cap \Locs^{\loosestrategy}$ we have 
	$\dhamm(\loc, \loc') = 1$. In particular,~\ref{item:counterfact-game_dHamm-1} 
	holds. And by taking any vertex of $\Locs_n \cap \Locs^{\loosestrategy}$ we 
	obtain~\ref{item:counterfact-game_dHamm-2}. 
	
	Now, we suppose that the properties hold for $i > 0$, and we suppose that 
	$\winplay = \loc \winplay'$ with $\loc \in \Locs_{n-i-1} \setminus 
	\Locs^{\loosestrategy}$. By definition of $\widetilde{\game}$, 
	$\weight(\winplay) = 1 + \weight(\winplay')$. By applying hypothesis of 
	induction~\ref{item:counterfact-game_dHamm-1} on $\winplay'$, we obtain for 
	all $\looseplay'$ be a \loosestrategy-play starting in $\Locs_{n - i}$ that 
	$\weight(\winplay) \leq 1 + \dhamm(\looseplay', \winplay')$. Since 
	$\loc \notin \Locs^{\loosestrategy}$, for all $\looseplay = \loc'\looseplay'$ be 
	a \loosestrategy-play from $\Locs_{n-i-1} \cap \Locs^{\loosestrategy}$, we have 
	$\dhamm(\looseplay, \winplay) = 1 + \dhamm(\looseplay', \winplay')$. In 
	particular, we conclude that~\ref{item:counterfact-game_dHamm-1} holds. Now, 
	to conclude~\ref{item:counterfact-game_dHamm-2}, we remark this hypothesis 
	of induction ensures us that there exists $\looseplay'$ be a \loosestrategy-play 
	starting in $\Locs_{n - i}$ such that $\weight(\winplay) = 1 + 
	\dhamm(\looseplay', \winplay')$. In particular, by fixing $\looseplay = 
	\loc'\looseplay'$ be a \loosestrategy-play from $\Locs_{n-i-1} \cap 
	\Locs^{\loosestrategy}$ (for any $\loc' \in \Locs^{\loosestrategy}$), we 
	have $\dhamm(\looseplay, \winplay) = 1 + \dhamm(\looseplay', \winplay')$ 
	and~\ref{item:counterfact-game_dHamm-2}.

	Finally, we suppose that $\winplay = \loc \winplay'$ with $\loc \in 
	\Locs_n \cap \Locs^{\loosestrategy}$. Again by definition of 
	$\widetilde{\game}$, $\weight(\winplay) = \weight(\winplay')$. By applying 
	hypothesis of induction~\ref{item:counterfact-game_dHamm-1} on $\winplay'$, 
	for all $\looseplay'$ be a \loosestrategy-play from $\Locs_{n-i}$ we have  
	$\weight(\winplay') \leq \dhamm(\looseplay', \winplay')$. Moreover, for all 
	$\looseplay = \loc' \looseplay'$ be a \loosestrategy-play from 
	$\Locs_{n-i-1} \cap \Locs^{\loosestrategy}$, 
	$\dhamm(\looseplay', \winplay') \leq \dhamm(\looseplay, \winplay)$: either 
	$\loc = \loc'$ and $\dhamm(\looseplay, \winplay) = \dhamm(\looseplay', 
	\winplay')$, or $\loc \neq \loc'$ and $\dhamm(\looseplay, \winplay) = 1 + 
	\dhamm(\looseplay', \winplay')$. Thus,~\ref{item:counterfact-game_dHamm-1} 
	holds. 

	Now, to conclude~\ref{item:counterfact-game_dHamm-2}, we remark this 
	hypothesis of induction ensures us that there exists $\looseplay'$ be a 
	\loosestrategy-play starting in $\Locs_{n - i}$ such that $\weight(\winplay) =  
	\dhamm(\looseplay', \winplay')$. Since $\loc \in \Locs_{n-i-1} \cap 
	\Locs^{\loosestrategy}$, we fix $\looseplay = \loc\looseplay'$
	\todo[inline]{Jakob: Why is this a play in the game. Is it not possible that the first state of $\looseplay'$ is not a successor of $\loc$?}
	 be a 
	\loosestrategy-play from $\Locs_{n-i-1} \cap \Locs^{\loosestrategy}$ such that 
	$\dhamm(\looseplay, \winplay) = \dhamm(\looseplay', \winplay')$ 
	and~\ref{item:counterfact-game_dHamm-2}. That conclude the proof by induction. 
	
	To conclude the proof of the lemma, we remark that 
	by~\ref{item:counterfact-game_dHamm-1}, for all \looseplay be a 
	\loosestrategy-play (from $\locinit$), we have 
	$\weight(\winplay) \leq \dhamm(\looseplay, \winplay)$. In particular, 
	(by definition of the infimum) $\weight(\winplay) \leq 
	\inf_{\looseplay \mid \text{\loosestrategy-play}} \, 
	\dhamm(\looseplay, \winplay)$. Moreover, since 
	by~\ref{item:counterfact-game_dHamm-2}, there exists \looseplay be a 
	\loosestrategy-play such that $\weight(\winplay) = \dhamm(\looseplay, \winplay)$, 
	we deduce that $\weight(\winplay) = 
	\inf_{\looseplay \mid \text{\loosestrategy-play}} \,
	\dhamm(\looseplay, \winplay)$.
	\qed
\end{proof}


\begin{lemma}
	\label{lem:counterfact-game_dHamm-2}
	Let \winstrategy be a winning strategy for \MinPl in $\widetilde{\game}$ (i.e. 
	for \SafePl in \game). Then, for all \looseplay be a \loosestrategy-play reaching 
	$\Locs_n$, there exists \winplay be a \winstrategy-play such that there 
	exists \play be a \winstrategy-play such that 
	\begin{displaymath}
	\weight(\play) \geq \dhamm(\looseplay, \winplay).
	\end{displaymath}
	\markend
\end{lemma}
\begin{proof}
	We reason by induction on $i$ (be the length of \loosestrategy-plays reaching 
	$\Locs_n$), to prove that for all \looseplay be a \loosestrategy-play from 
	$\Locs_{n-i}$ such that there exists \winplay be a \winstrategy-play from 
	$\loc \in \Locs_{n-i}$, there exists \play be a \winstrategy-play from 
	$\loc \in \Locs_{n-i}$ such that 
	$\weight(\play) \geq \dhamm(\looseplay, \winplay)$.
	
	First, we suppose that $i = 0$ and we let $\loc \in \Locs_n$ be a 
	\loosestrategy-play. We fix $\looseplay = \loc = \strategy$ that are  
	\winstrategy-plays such that $\dhamm(\loc, \looseplay) = 0$. Since 
	$\widetilde{\game}$ contains only non-negative weight, we have 
	$\weight(\play) \geq 0$. In particular, the property holds for $i=0$.
	
	Now, we suppose that $i \geq 0$ and we suppose that the property holds for $i$.  
	We let $\looseplay = \loc \looseplay'$ be a \loosestrategy-play from 
	$\Locs_{n-i-1}$ reaching $\Locs_n$. Now, we fix $\winplay = \loc \winplay'$ be 
	a \winstrategy-play. In particular, $\dhamm(\play, \looseplay) = 
	\dhamm(\play', \looseplay')$ (since the first vertices of both plays are the 
	same). By applying hypothesis of induction in $\looseplay'$ and 
	$\winplay'$, there exists $\play'$ from $\loc' \in \Locs_{n-i}$ the first 
	vertex of $\winplay'$ such that $\weight(\play') \geq 
	\dhamm(\looseplay', \winplay')$. Since \winplay is a \winstrategy-play, 
	$\play = \loc \play'$ is a \winstrategy-play too (i.e. 
	$\winstrategy(\loc) = (\loc, \loc')$ by definition of \winplay). 
	Moreover, since $\widetilde{\game}$ are only non-negative weight, 
	$\weight(\winplay) \geq \weight(\winplay')$. Thus, 
	we deduce that  
	\begin{displaymath}
	\weight(\play) \geq \weight(\play') \geq \dhamm(\winplay', \looseplay') = 
	\dhamm(\winplay, \looseplay).
	\end{displaymath}
	\qed
\end{proof}

Now, we prove that the cost of a strategy \winstrategy encodes its Hausdorff-Hamming 
distance with \loosestrategy, i.e. we prove 
Proposition~\ref{prop:counterfact-game_dHamm}.

\begin{proof}[Proof of Proposition~\ref{prop:counterfact-game_dHamm}]
	First, we rewrite the equality by 
	\begin{displaymath}
	\sup_{\substack{\strategy \\ \text{strategy of \SafePl}}} 
	\weight(\outcomes(\locinit, \winstrategy, \strategy)) = 
	\max 
	\begin{cases}
	\sup_{\looseplay \mid \text{\loosestrategy-play}} \,
	\inf_{\winplay \mid \text{\winstrategy-play}} \,
	\dhamm(\looseplay, \winplay) \\
	\sup_{\winplay \mid \text{\winstrategy-play}} \,
	\inf_{\looseplay \mid \text{\loosestrategy-play}} \,
	\dhamm(\looseplay, \winplay) 
	\end{cases}
	\end{displaymath}
	with the definition of the cost of \winstrategy and the Hausdorff-Hamming 
	distance. Now, we deduce that 
	$\sCost(\winstrategy) \leq \dhamm^H(\loosestrategy, \winstrategy)$ from  the 
	following property
	\begin{displaymath}
	\sCost(\winstrategy)
	= \sup_{\winplay \mid \winstrategy-play} \,
	\inf_{\looseplay \mid \text{\loosestrategy-play}} \,
	\dhamm(\looseplay, \winplay).
	\end{displaymath}
	To prove it, we apply Lemma~\ref{lem:counterfact-game_dHamm-1}, we deduce that 
	for all \winplay be a \winstrategy-play, we have $\weight(\winplay) = 
	\inf_{\looseplay \mid \text{\loosestrategy-play}} \, 
	\dhamm(\looseplay, \winplay)$. When we fix one strategy by players, we 
	obtain only one play that is conforming to both strategies. In particular, 
	computing the supremum over all \winstrategy-plays consists of computing the 
	supremum over all strategies of \SafePl. Thus, 
	$\sCost(\winstrategy) = \sup_{\winplay \mid \winstrategy-play} \,
	\inf_{\looseplay \mid \text{\loosestrategy-play}} \, 
	\dhamm(\looseplay, \winplay)$, by applying the supremum in both terms of equality.
	
	Conversely, we prove that $\sCost(\winstrategy) \geq 
	\dhamm^H(\loosestrategy, \winstrategy)$. In particular, by the previous 
	item, we prove that $\sCost(\winstrategy) \geq 
	\sup_{\looseplay \mid \text{\loosestrategy-play}} 
	\inf_{\winplay \mid \text{\winstrategy-play}} \dhamm^H(\looseplay, \winplay)$.
	In particular, by definition of the supremum, we need to prove that 
	for all \looseplay be a \loosestrategy-play, $\sCost(\winstrategy) \geq 
	\inf_{\winplay \mid \text{\winstrategy-play}} \dhamm^H(\looseplay, \winplay)$. 
	Moreover, by definition of the infimum, we need to prove that for all \looseplay 
	be a \loosestrategy-play, there exists \winplay be a \winstrategy-play such that 
	$\sCost(\winstrategy) \geq  \dhamm^H(\looseplay, \winplay)$. Finally, by 
	definition of \sCost, we need to prove that  for all \looseplay 
	be a \loosestrategy-play, there exists \winplay be a \winstrategy-play such that 
	there exists \play by a \winstrategy-play such that $\weight(\play) \geq  
	\dhamm^H(\looseplay, \winplay)$. Thus, we conclude by applying 
	Lemma~\ref{lem:counterfact-game_dHamm-2}.
	\qed
\end{proof}

Now, we have tools to prove the Theorem~\ref{thm:check-counterfactual-game}.

\begin{proof}[Proof of Theorem~\ref{thm:check-counterfactual-game}]
	The algorithm to test the last condition contains three steps:
	\begin{enumerate}
		\item computing the first shortest-path game $\widetilde{\game}_1$ that 
		is $\widetilde{\game}$ where we have removed all vertices of $C$, 
		and we compute $\winstrategy^1$ be an optimal strategy for \MinPl in 
		$\widetilde{\game}_1$ (i.e. for \SafePl in \game);
		\item computing the second shortest-path game $\widetilde{\game}_2$ that 
		is $\widetilde{\game}_1$ where we change the target of the game, i.e. 
		$\Locs_T = \LocsNegT$ in $\widetilde{\game}_2$. Then, we compute 
		$\winstrategy^2$ be an optimal strategy for \MinPl in $\widetilde{\game}_2$; 
		\item comparing the cost of both strategies.
	\end{enumerate}
	We remark that each step of this algorithm is computed in polynomial time since 
	computing $\winstrategy^1$ and $\winstrategy^2$ is given in polynomial time (see 
	Proposition~\ref{prop:SPG-solve}).

	To conclude the proof, we prove its correction, i.e. 
	$\sCost(\winstrategy^1) < \sCost(\winstrategy^2)$ if and only if $C$ is a 
	$\dhamm^H$-contrafactual cause. In particular, since $\winstrategy^1$ is an 
	optimal strategy in $\widetilde{\game}_1$, by 
	Lemma\ref{lem:counterfact-game_dHamm} it minimises the Hausdorff-Hamming distance 
	with \loosestrategy for strategies of \SafePl. Moreover, by definition of 
	$\widetilde{\game}_1$ and \game, $\winstrategy^1$ is a winning strategy of 
	\SafePl in \game that avoids $C$. By the same arguments in $\widetilde{\game}_2$, 
	$\winstrategy^2$ minimises $\dhamm^H$ with \loosestrategy for non-winning 
	strategies of \SafePl (since reach a vertices of \LocsNegT is the unique way to 
	\SafePl to win in \game by hypothesis on it) that avoids $C$.
	\qed
\end{proof}




\subsection{Counterfactual causes for further distance functions on MD-strategies?}







==> sections/app_quasi-cause-checking.tex <==
\section{Proof of Theorem~\ref{thm:dkstrat-cause_check}}
\label{app:quasi-cause-checking.tex}

\todo[inline]{To review according the new Thm. 9}
In this appendix, we make the detailed proof of Theorem~\ref{thm:dkstrat-cause_check}. 
\dkcauseCheck*

A $k,d$-cause is checking in polynomial time since we can check in polynomial time 
quasi-strat-cause. In particular, we have the following property.




Before to conclude the proof of Theorem~\ref{thm:dcause_check}, in the case of $C$ is a 
quasi-strat-cause, we need to prove that there exists a $C$-cause strategy \winstrategy such that 
$d(\winstrategy, \loosestrategy) \leq k$ for Hamming and \dHH distances.

\begin{proposition}
	\label{prop:dcause_check-dist}
	Let \winstrategy be a $C$-cause strategy. Then, Hamming and \dHH distances of \winstrategy 
	and \loosestrategy are upper-bound by size of $C$, i.e. 
	$\dhamm(\loosestrategy, \winstrategy) \leq |C|$ and 
	$\dHH(\loosestrategy, \winstrategy) \leq |C|$.
\end{proposition}
\begin{proof}
	First, we prove that $\dhamm(\loosestrategy, \winstrategy) \leq |C|$. To do that, we apply 
	the definition of $\dhamm$: $\dhamm(\loosestrategy, \winstrategy) = |\{\loc \mid 
	\loosestrategy(\loc) \neq \winstrategy(\loc)\}|$. Since \winstrategy be a $C$-cause 
	strategy, $\{\loc \mid \loosestrategy(\loc) \neq \winstrategy(\loc)\} = C$. Thus, 
	$\dhamm(\loosestrategy, \winstrategy) = |C|$.
	
	To conclude the proof, we prove that $\dHH(\loosestrategy, \winstrategy) \leq |C|$.
	By definition of \dHH, the distance computes along all \winstrategy-plays and 
	\loosestrategy-plays the number of vertices where \loosestrategy and \winstrategy are 
	distinct (and not their occurrence). In particular, in the worst case a play go through 
	all vertices of \game. Moreover, since \winstrategy be a $C$-cause strategy, $C = 
	\{\loc \mid \loosestrategy(\loc) \neq \winstrategy(\loc)\}$. Thus, 
	$\dHH(\loosestrategy, \winstrategy) \leq |C|$.
	\qed
\end{proof}



==> sections/app_quasi-cause-find.tex <==
\section{Proof of Theorem~\ref{thm:dstrat-cause_check}}
\label{app:quasi-cause-find}



\todo[inline]{Below (in red) copied from main paper!!!! to be removed!!!}


\textcolor{red}{
Letting a reachability game \game where \Pl wins, a non-winning MD-strategy 
\loosestrategy for \Pl, a distance for MD-strategies $d$ and a potential cause $C$, 
we want to check if $C$ is $d$-strat-cause. In particular, by guessing $k$ be the 
minimal distance for a winning MD-strategy to \loosestrategy, we can 
check if $C$ is a $k,d$-strat-cause in polynomial time for the Hamming strategy 
distance and \dHH (by Theorem~\ref{thm:dkstrat-cause_check}). Thus, the problem is in 
NP for all both distances and players. Moreover, we prove that this problem is 
NP-complete under $\dhamm^s$ for \ReachPl since finding a winning MD-strategy that 
minimises $\dhamm^s$ is NP-complete (by Theorem~\ref{thm:strat_finding-NP-c}). }

\begin{restatable}{theorem}{dkcauseCheck}
	\label{thm:dkstrat-cause_check}
\textcolor{red}{	Let \game be a reachability game where \Pl wins, \loosestrategy be a non-winning 
	MD-strategy for \Pl, $d$ a distance over MD-strategies, $k \in \N$ and a 
	potential cause $C \subseteq \Locs$. We can check if $C$ is a $k,d$-strat-cause 
	in polynomial time when $d$ is the Hamming strategy distance or \dHH. }
\end{restatable}
\begin{proof}[Sketch of proof]
\textcolor{red}{	The algorithm to check when a candidate cause $C$ is a $k,d$-strat-cause for 
	$\dhamm^s$ or \dHH consists in four steps. The first one removes in \game all 
	edges given by $\loosestrategy(\loc)$ when $\loc \in C$. Then, we build the 
	reachability game under \loosestrategy from this new game, denoted 
	$\game^{\loosestrategy}$. Next, we test the existence of a winning 
	MD-strategy for \Pl in $\game^{\loosestrategy}$, thus we check if $C$ is a 
	quasi-strat-cause. Finally, we check if the size of $C$ is less than $k$ since we 
	prove that the distance of a $C$-distinct \loosestrategy-strategy to 
	\loosestrategy are upper-bound by the size of $C$. To conclude, we remark that 
	each step can be done in polynomial time. The detailed proof is given in 
	Appendix~\ref{app:quasi-cause-checking.tex}. }
	\qed
\end{proof}

\textcolor{red}{
Theorem~\ref{thm:dkstrat-cause_check} does not prove that the checking cause problem 
for Hamming strategy distance and \dHH is solved in polynomial time. Moreover, we 
prove that the problem of checking a $\dhamm^s$-strat-cause is NP-complete for 
\ReachPl.}



In this appendix, we makes the detailed proof of Theorem~\ref{thm:dstrat-cause_check}.

\dcauseCheck*

To prove this theorem, we will focus on the decision problem. In particular, we 
focus on the problem of checking whether $C$ is \emph{ a $k, \dhamm^s$-strat-cause}, i.e. whether $C$ is a 
quasi-strat-cause such that there exists   a $C$-distinct \loosestrategy-strategy  \winstrategy
with $\dhamm^s(\winstrategy, \loosestrategy) \leq k$.

First, we prove the NP-easiness of the problem of checking if $C$ is a 
$\dhamm^s$-strat-cause. In particular, we prove that checking if $C$ is 
a quasi-strat-cause in polynomial time. Then, we guess a $C$-distinct 
\loosestrategy-strategy such that $\dhamm^s(\winstrategy, \loosestrategy) \leq k$ 
(it is testable in polynomial time since we can compute 
$\dhamm^s$ in polynomial time because it just counts positions at which the strategies differ). Moreover, we prove that checking a quasi-strat-cause in polynomial 
time is done for both players. 

\paragraph{Checking quasi-strat-cause.} 
The NP-easiness of this problem consists on the proof of the checking quasi-strat-cause. 
Intuitively, it is possible to check if the partial MD-strategy that is not defined 
on vertices of $C$ defines a reachability game where \Pl wins. 

\begin{proposition}
	\label{prop:dcause_check-quasi}
	Let \game be a reachability game where \Pl wins, \loosestrategy be a non-winning 
	MD-strategy for \Pl, and a potential cause $C \subseteq \Locs$. We can check 
	if $C$ is a quasi-strat-cause in polynomial time. 
\end{proposition}

Recall, to check if $C$ is quasi-strat-cause, we define \strategy be a partial strategy such 
that it makes same choices of \loosestrategy for vertices are not in $C$. Then, we check if 
\Pl wins in $\game^{\strategy}$. In particular, we prove the utility of $\game^{\strategy}$ to 
check the potential cause. 

\begin{lemma}
	\label{lem:check-win-cause}
	Let $\game$ be a reachability game with a (partial) strategy \loosestrategy 
	for \Pl. 
	\begin{enumerate}
		\item\label{item:check-win-cause_pos} If \Pl wins in $\game^{\loosestrategy}$, then 
		there exists \winstrategy a winning strategy in \game such that 
		$\winstrategy(\loc) = \loosestrategy(\loc)$ when \loosestrategy is defined.
		\item\label{item:check-win-cause_neg} If \Pl loses in  $\game^{\loosestrategy}$, then 
		all strategies \strategy in \game such that $\strategy(\loc) = \loosestrategy(\loc)$ 
		when \loosestrategy is defined are non-winning.
	\end{enumerate}
\end{lemma}
\begin{proof}
	\begin{enumerate}
		\item We suppose that \Pl wins in $\game^{\loosestrategy}$, i.e. there exists a winning 
		strategy \winstrategy in $\game^{\loosestrategy}$. By definition of 
		$\game^{\loosestrategy}$, when \loosestrategy is define, $\loosestrategy(\loc)$ is the 
		only choice of \Pl in \loc. Thus, $\winstrategy(\loc) = \loosestrategy(\loc)$ 
		when \loosestrategy is defined. To conclude this item, we prove that all 
		\winstrategy-plays in \game are also a \winstrategy-play in $\game^{\loosestrategy}$.
		Let \winplay be a \winstrategy-play in \game and we reason by induction on length 
		of \winplay. If $\winplay = \loc$, then \loc is also a \winstrategy-play in 
		$\game^{\loosestrategy}$ since their vertices are exactly the same as ones of \game.
		Now, we suppose that $\winplay = \loc\winplay'$ be a \winstrategy-play in \game with 
		$\loc'$ the first vertex of $\winplay'$. By hypothesis of induction $\winplay'$ is 
		a \winstrategy-play in $\game^{\loosestrategy}$. To conclude, we check if 
		$(\loc, \loc') \in \Trans^{\loosestrategy}$ according the belong of \loc. If 
		$\loc \notin \Locs_{\Pl}$, then $(\loc, \loc') \in \Trans^{\loosestrategy}$ since 
		$\game^{\loosestrategy}$ does not remove edges of the opponent of $\Pl$. Otherwise, 
		$\loc \in \Locs_{\Pl}$ and $(\loc, \loc') \in \Trans^{\loosestrategy}$ since 
		\winstrategy is a strategy of $\game^{\loosestrategy}$. 		
		
		\item We suppose that \Pl loses in $\game^{\loosestrategy}$, and 
		we reason by contradiction. We suppose that there exists a winning 
		strategy \winstrategy in \game such that 
		$\winstrategy(\loc) = \loosestrategy(\loc)$ when \loosestrategy is 
		defined. In particular, we remark that \winstrategy is a strategy 
		in $\game^{\loosestrategy}$ (since \winstrategy chooses the unique 
		choice of \loc in $\game^{\loosestrategy}$ when \loosestrategy is 
		defined). Since $\game^{\loosestrategy}$ is a sub-game of \game, 
		\winstrategy is a winning strategy in $\game^{\loosestrategy}$. Thus, 
		\Pl wins in $\game^{\loosestrategy}$.
		\qed
	\end{enumerate}
\end{proof}

Now, we have the tools to prove Proposition~\ref{prop:dcause_check-quasi}.
\begin{proof}[Proof of Proposition~\ref{prop:dcause_check-quasi}]
	We begin by defining a partial strategy \strategy from \loosestrategy to remove choices 
	of vertices of $C$. Formally, for all $\loc \in \Locs_{\Pl} \setminus C$, we define 
	\strategy such that $\strategy(\loc) = \loosestrategy(\loc)$ and we test if \Pl wins in 
	$\game^{\strategy}$. If \Pl wins, then there exists \winstrategy be a winning 
	strategy in \game such that $\winstrategy(\loc) = \loosestrategy(\loc)$ if and only if 
	$\loc \notin C$ (by Lemma~\ref{lem:check-win-cause}.\ref{item:check-win-cause_pos}). Thus, 
	$C$ is a quasi-strat-cause. Conversely, if \Pl loses, then all strategies \winstrategy in \game 
	such that $\winstrategy(\loc) = \loosestrategy(\loc)$ if and only if $\loc \notin C$
	are non-winning (by Lemma~\ref{lem:check-win-cause}.\ref{item:check-win-cause_neg}). 
	Thus, $C$ is not a quasi-strat-cause. 
	
	Now, to conclude the proof, we remark that \strategy is only a filter of \loosestrategy, 
	and $\game^{\strategy}$ is a filter of edges of \game. Thus, $\game^{\strategy}$ is 
	computable in polynomial time and its size is less than one of \game. Moreover, deciding 
	if \Pl wins in a reachability game is done in polynomial time in size of this game 
	(by \cite{GradelTW-02}). In particular, we decide in polynomial time on size of \game 
	if \Pl wins in $\game^{\strategy}$.
	\qed
\end{proof}


Finally, to prove Theorem~\ref{thm:dstrat-cause_check}, we want to prove the NP-hardness 
of the checking problem for $k,\dhamm^s$-strat-cause. To do that, we reduce into the 
problem to finding a winning MD-strategy \winstrategy such that 
$\dhamm^s(\winstrategy, \loosestrategy) \leq k$ that is an NP-complete (by 
Theorem ~\ref{thm:strat_finding-NP-c}). The main argument of this reduction is the 
proof that we can compute a quasi-strat-cause in polynomial time.

\paragraph{Computing a quasi-strat-cause.}
Now, we want to check if there exists a quasi-strat-cause in \game under \loosestrategy. 
Since we have just proved that checking a potential cause $C$ is done in polynomial time 
(see Proposition~\ref{prop:dcause_check-quasi}), testing the existence of a quasi-strat-cause is 
in NP: we guess a potential cause $C$, and we check in polynomial time if $C$ is well a 
quasi-strat-cause. However, we improve this result by proving that we can compute a quasi-strat-cause 
in polynomial time for both players.

\begin{proposition}
	\label{prop:game_find}
	Let \game be a reachability game where \Pl wins and \loosestrategy be a 
	non-winning strategy for \Pl. Testing the existence of a quasi-strat-cause and computing 
	it (when exists) can be done in polynomial time. 
\end{proposition}

Intuitively a non-winning MD-strategy for \ReachPl chooses a wrong 
edge, i.e. it quit the attractor to the effect. In particular, a quasi-strat-cause 
is given by the set of choices of \loosestrategy that quit the attractor. 
Formally, we prove that 
\begin{equation}
\label{eq:c-Reach}
C_{\ReachPl} = \{\loc \mid \loosestrategy(\loc) \in \Trans^\loosestrategy \setminus 
\Trans^*_{\LocsT} \}
\end{equation}
is a quasi-strat-cause (when a quasi-strat-cause exists) for \ReachPl. By a same 
reasoning, wrong edges chosen by a non-winning MD-strategy for \SafePl 
reach the attractor to the effect. In particular, 
\begin{equation}
\label{eq:c-Safe}
C_{\SafePl} = \{\loc \mid 
\loosestrategy(\loc) = (\loc, \loc') \text{ with } \loc \in \Locs^\loosestrategy 
\cap \Locs^*_{\LocsT} \}
\end{equation}
is a quasi-strat-cause (when a quasi-strat-cause exists) for \SafePl. Thus, as 
attractor can be computed in polynomial time (by \cite{GradelTW-02}), the 
existence of a quasi-strat-cause is done in polynomial time. We start by the point 
of view of \ReachPl.


\begin{proposition}
	\label{prop:find-win_Reach}
	Let \game be a reachability game where \ReachPl wins, and \loosestrategy 
	be a non-winning strategy for \ReachPl. Then, $C_{\ReachPl}$ defined 
	in~\eqref{eq:c-Reach} is a quasi-stat-cause for \game under \loosestrategy.
\end{proposition}

An important tool of the proof of this proposition is the fact that  
inside a reachability game defined by an attractor to the effect, all edges from 
a vertex of \ReachPl define a winning MD-strategy. In particular, we can change  
choices of a winning MD-strategy as long as these new choices belong to the attractor.
Formally, we have the following Lemma:
\begin{lemma}
	\label{lem:attractor_strat} 
	Let \game be a reachability game where \ReachPl wins. We fix 
	$\game_{\LocsT} = (\Locs^*_{\LocsT}, \locinit, \Trans^*_{\LocsT})$ be a 
	reachability game computed by an attractor to \LocsT in \game, 
	\winstrategy be a winning MD-strategy in $\game_{\LocsT}$, and 
	$(\loc_1, \loc_2) \in \Trans^*_{\LocsT}$. We define \strategy be a MD-strategy 
	in \game such that, for all vertices $\loc'' \in \LocsReach$,
	\begin{displaymath}
	\strategy(\loc) = 
	\begin{cases}
	\loosestrategy(\loc) & \text{if $\loc \neq \loc_1$;} \\
	(\loc_1, \loc_2) & \text{otherwise.}
	\end{cases}
	\end{displaymath}
	Then, \strategy is a winning MD-strategy.
\end{lemma}
\begin{proof}
	We reason by contradiction, and we suppose that \strategy is not winning.
	In particular, we suppose that there exits \play be a \strategy-play such 
	that \play does not reach \LocsT, and we distinguish two cases. First, we 
	suppose that \play is acyclic, i.e. $|\play| \leq |\Locs|$. Like, 
	\play does not reach \LocsT, we know that $\loc \in \play$, 
	otherwise \play reaches the effect (since \play is also a \winstrategy-play). 
	Moreover, from $\loc'$, we know that \play is a \winstrategy-play (by 
	definition of \strategy, and since \play is acyclic). 
	Thus, \play reaches \LocsT.
	
	Now, we suppose that \play contains a cycle that we denote $c$. If there exist 
	$(\loc, \loc') \in c$ such that $\loc \in \Locs^n_{\LocsT}$ for some $n$, and 
	$\loc' \in \Locs^{n+1}_{\LocsT}$, then it is impossible by definition of 
	$\Trans^{n}_{\LocsT}$. Otherwise, for all $(\loc, \loc') \in c$, if 
	$\loc \in \Locs^n_{\LocsT}$ for some $n$, then $\loc' \in \Locs^n_{\LocsT}$. 
	In particular, there exists $(\loc, \loc')$ such that $(\loc, \loc') \notin 
	\Trans^*_{\LocsT}$ that is impossible by definition of \strategy (that use 
	only choices of \winstrategy be a strategy in $\game^{\loosestrategy}$ and 
	$(\loc_1,\loc_2) \in \Trans^*_{\LocsT}$ by hypothesis). Thus, \play is acyclic. 
	\qed
\end{proof}

To prove Proposition~\ref{prop:find-win_Reach}, we prove that $C_{\ReachPl}$ is a 
quasi-strat-cause when it is non-empty with the previous lemma.

\begin{lemma}
	\label{lem:find-win_trans}
	If $C_{\ReachPl} \neq \emptyset$, then $C_{\ReachPl}$ is a quasi-strat-cause.
\end{lemma}
\begin{proof}
	Since \ReachPl wins in \game, we consider \winstrategy be a winning 
	MD-strategy for \ReachPl. If for all vertices $\loc \in \LocsReach$, we have 
	$\winstrategy(\loc) = \loosestrategy(\loc)$ if and only if 
	$\loosestrategy(\loc) \notin C_{\ReachPl}$, then $C_{\ReachPl}$ is a 
	quasi-strat-cause .
	
	Otherwise, we suppose that there exists a vertex $\loc \in \LocsReach$ such 
	that $\loosestrategy(\loc) \notin C_{\ReachPl}$, but $\winstrategy(\loc) \neq 
	\loosestrategy(\loc)$, and we let $L(\winstrategy)$ be this set of vertices. 
	Since $\loosestrategy(\loc) \notin C_{\ReachPl}$, the chosen edge is 
	necessarily in $\Trans^*_{\LocsT}$, i.e. 
	$\loosestrategy(\loc) \in \Trans^*_{\LocsT}$. Then, by induction on the size 
	of $|L(\winstrategy)|$, that there exists a winning MD-strategy \strategy such 
	that the size of $L(\strategy)$ strictly decrease. More precisely, let 
	$\loc \in L(\winstrategy)$, then we fix \strategy be a MD-strategy such that, 
	for all $\loc'' \in \LocsReach$, 
	\begin{displaymath}
	\strategy(\loc'') = 
	\begin{cases}
	\loosestrategy(\loc'') & \text{if $\loc'' \neq \loc$} \\
	(\loc, \loc') & \text{otherwise}
	\end{cases}
	\end{displaymath}
	with $(\loc, \loc') \in \Trans^*_{\LocsT}$. Thus, by 
	Lemma~\ref{lem:attractor_strat}, \winstrategy is a winning MD-strategy. By 
	induction, we define a winning MD-strategy \winstrategy such that if 
	$\loosestrategy(\loc) \notin C_t$, then $\winstrategy(\loc) = 
	\loosestrategy(\loc)$.
	
	To conclude, we suppose that there exists a vertex $\loc \in \LocsReach$ 
	such that $\winstrategy(\loc) = \loosestrategy(\loc)$, but 
	$\loosestrategy(\loc) \in C_{\ReachPl}$. However, since \winstrategy is a 
	winning MD-strategy, we can apply Lemma~\ref{lem:attractor_strat} to change 
	the choice of \loc in \winstrategy. In particular, we obtain a 
	winning MD-strategy \winstrategy such that $\winstrategy(\loc) = 
	\loosestrategy(\loc)$ if and only if $\loosestrategy(\loc) \notin 
	C_{\ReachPl}$.
	\qed
\end{proof}

Now, we conclude the proof of Proposition~\ref{prop:find-win_Reach}.

\begin{proof}[Proof of Proposition~\ref{prop:find-win_Reach}]
	To conclude the proof, we prove that $C_{\ReachPl} \neq \emptyset$.
	In particular, we reason by contradiction, and we suppose that 
	$C_{\ReachPl} = \emptyset$. By hypothesis \ReachPl wins in \game, so 
	$\locinit \in \Locs^*_{\LocsT}$. Thus, \ReachPl wins in 
	$(\Locs^*_{\LocsT}, \locinit, \Trans^*_{\LocsT})$. Since \loosestrategy is 
	a non-winning MD-strategy of \ReachPl, there exists $\loc \in \LocsReach$ 
	such that $\loosestrategy(\loc) = (\loc, \loc') \notin \Trans^*_{\LocsT}$ 
	(otherwise, all choices of \loosestrategy is in $\Trans^*_{\LocsT}$, then 
	by Lemma~\ref{lem:attractor_strat}, \loosestrategy is a winning MD-strategy). 
	Thus, by~\eqref{eq:c-Reach}, $(\loc, \loc') \in C_{\ReachPl}$ since 
	$\loc' \in \Locs^{\loosestrategy}$ and $C_{\ReachPl} \neq \emptyset$. 
	\qed
\end{proof}

Now, we focus on point of view of \SafePl. In particular, we make an 
analogous reasoning.

\todo[inline]{To review}
\begin{proposition}
	\label{prop:find-win_Safe}
	Let \game be a reachability game where \SafePl wins, and \loosestrategy 
	be a non-winning MD-strategy for \SafePl. Then, $C_{\SafePl}$ defined 
	by~\eqref{eq:c-Safe} is a quasi-strat-cause for \game under \loosestrategy.
\end{proposition} 

An important tool of the proof of this proposition is the fact that  
inside a reachability game defined from an attractor to the effect, all edges from 
a vertex of \SafePl define a winning MD-strategy. In particular, we can change  
choices of a winning MD-strategy as long as these new choices avoid the attractor.
Formally, we have the following Lemma:
\begin{lemma}
	\label{lem:attractor_strat-Safe} 
	Let \game be a reachability game where \SafePl wins. We fix 
	$\game_{\LocsT} = (\Locs \setminus \Locs^*_{\LocsT}, \locinit, 
	\Trans \setminus \Trans^*_{\LocsT})$ be a reachability game computed from 
	an attractor to \LocsT in \game, \winstrategy be a winning MD-strategy in 
	$\game_{\LocsT}$, and $(\loc_1, \loc_2) \in \Trans \setminus 
	\Trans^*_{\LocsT}$. We define \strategy be a MD-strategy in \game such 
	that, for all vertices $\loc'' \in \LocsReach$,
	\begin{displaymath}
	\strategy(\loc) = 
	\begin{cases}
	\loosestrategy(\loc) & \text{if $\loc \neq \loc_1$;} \\
	(\loc_1, \loc_2) & \text{otherwise.}
	\end{cases}
	\end{displaymath}
	Then, \strategy is a winning MD-strategy.
\end{lemma}
\begin{proof}
	We reason by contradiction, and we suppose that \strategy is not winning.
	In particular, we suppose that there exits \play be a \strategy-play such 
	that \play reaches \LocsT. In particular, \play is acyclic (since both 
	strategies are memoryless), i.e. $|\play| \leq |\Locs|$. Like, 
	\play does reaches \LocsT, we know that $\loc \in \play$, otherwise \play 
	avoids the effect (since \play is also a \winstrategy-play). 
	Moreover, from $\loc'$, we know that \play is a \winstrategy-play (by 
	definition of \strategy, and since \play is acyclic). 
	Thus, \play does not reach \LocsT. 
	\qed
\end{proof}

To prove Proposition~\ref{prop:find-win_Safe}, we prove that $C_{\SafePl}$ 
is a quasi-strat-cause when it is non-empty with the previous lemma.

\begin{lemma}
	\label{lem:find-win_trans-Safe}
	If $C_{\SafePl} \neq \emptyset$, then $C_{\SafePl}$ is a quasi-strat-cause.
\end{lemma}
\begin{proof}
	Since \SafePl wins in \game, we consider \winstrategy be a winning 
	MD-strategy for \SafePl. If for all vertices $\loc \in \LocsSafe$, we have 
	$\winstrategy(\loc) = \loosestrategy(\loc)$ if and only if 
	$\loosestrategy(\loc) \notin C_{\SafePl}$, then $C_{\SafePl}$ is a 
	quasi-strat-cause .
	
	Otherwise, we suppose that there exists a vertex $\loc \in \LocsSafe$ such 
	that $\loosestrategy(\loc) \notin C_{\SafePl}$, but $\winstrategy(\loc) \neq 
	\loosestrategy(\loc)$, and we let $L(\winstrategy)$ be this set of vertices. 
	Since $\loosestrategy(\loc) \notin C_{\SafePl}$, the chosen edge is 
	necessarily in $\Trans \setminus \Trans^*_{\LocsT}$, i.e. 
	$\loosestrategy(\loc) \in \Trans \setminus \Trans^*_{\LocsT}$. Then, by 
	induction on the size of $|L(\winstrategy)|$, that there exists a winning 
	MD-strategy \strategy such that the size of $L(\strategy)$ strictly decrease. 
	More precisely, let $\loc \in L(\winstrategy)$, then we fix \strategy be a 
	MD-strategy such that, for all $\loc'' \in \LocsSafe$, 
	\begin{displaymath}
	\strategy(\loc'') = 
	\begin{cases}
	\loosestrategy(\loc'') & \text{if $\loc'' \neq \loc$} \\
	(\loc, \loc') & \text{otherwise}
	\end{cases}
	\end{displaymath}
	with $(\loc, \loc') \in \Trans \setminus \Trans^*_{\LocsT}$. Thus, by 
	Lemma~\ref{lem:attractor_strat-Safe}, \winstrategy is a winning MD-strategy. 
	By induction, we define a winning MD-strategy \winstrategy such that if 
	$\loosestrategy(\loc) \notin C_{\SafePl}$, then $\winstrategy(\loc) = 
	\loosestrategy(\loc)$.
	
	To conclude, we suppose that there exists a vertex $\loc \in \LocsReach$ 
	such that $\winstrategy(\loc) = \loosestrategy(\loc)$, but 
	$\loosestrategy(\loc) \in C_t$. However, since \winstrategy is a winning 
	MD-strategy, we can apply Lemma~\ref{lem:attractor_strat} to change the 
	choice of \loc in \winstrategy. In particular, we obtain a 
	winning MD-strategy \winstrategy such that $\winstrategy(\loc) = 
	\loosestrategy(\loc)$ if and only if $\loosestrategy(\loc) \notin 
	C_{\ReachPl}$.
	\qed
\end{proof}

Now, we conclude the proof of Proposition~\ref{prop:find-win_Safe}.

\begin{proof}[Proof of Proposition~\ref{prop:find-win_Safe}]
	To conclude the proof, we prove that $C_{\SafePl} \neq \emptyset$.
	In particular, we reason by contradiction, and we suppose that 
	$C_{\SafePl} = \emptyset$. By hypothesis \SafePl wins in \game, so 
	$\locinit \in \Locs \setminus \Locs^*_{\LocsT}$. Thus, \SafePl wins in 
	$(\Locs \setminus \Locs^*_{\LocsT}, \locinit, 
	\Trans \setminus \Trans^*_{\LocsT})$. Since \loosestrategy is 
	a non-winning MD-strategy of \SafePl, there exists $\loc \in \LocsSafe$ 
	such that $\loosestrategy(\loc) = (\loc, \loc') \notin \Trans \setminus 
	\Trans^*_{\LocsT}$ (otherwise, all choices of \loosestrategy is in 
	$\Trans \setminus \Trans^*_{\LocsT}$, then by 
	Lemma~\ref{lem:attractor_strat-Safe}, \loosestrategy is a winning 
	MD-strategy). Thus, by~\eqref{eq:c-Safe}, $(\loc, \loc') \in C_{\SafePl}$ 
	since $\loc' \in \Locs^{\loosestrategy}$ and $C_{\SafePl} \neq \emptyset$. 
	\qed
\end{proof}


\paragraph{Reduction into the problem of finding a winning MD-strategy.} 
To conclude the proof of Theorem~\ref{thm:dstrat-cause_check}, we 
reduce the decision version of the problem of checking a 
$\dhamm^s$-strat-cause into the decision version of the problem of finding 
a winning MD-strategy for \ReachPl that minimises $\dhamm^s$ of 
\loosestrategy. Formally, let \game be a reachability game where 
\ReachPl wins, \loosestrategy be a non-winning MD-strategy for \ReachPl 
and $k \in \N$ a given threshold. From \game and \loosestrategy, we 
define a quasi-strat-cause $C_{\ReachPl}$ (defined by~\eqref{eq:c-Reach}), 
by Proposition~\ref{prop:find-win_Reach}. Now, we formally prove the 
correctness of this reduction. 

\begin{lemma}
	\label{lem:dstrat-cause-check_red}
	The two following properties are equivalent: 
	\begin{enumerate}
		\item $C_{\ReachPl}$ is a $k, \dhamm^s$-strat-cause;
		\item there exists \winstrategy be a winning MD-strategy for 
		\ReachPl such that $\dhamm^s(\loosestrategy, \winstrategy) \leq k$.
	\end{enumerate}
\end{lemma}
\begin{proof}
	We begin by supposing that $C_{\ReachPl}$ is a $k, \dhamm^s$-strat-cause. 
	In particular, by definition of a such cause, there exists \winstrategy be 
	a $C_{\ReachPl}$-distinct \loosestrategy-strategy, i.e. a winning MD-strategy 
	for \ReachPl, such that $\dhamm^s(\loosestrategy, \winstrategy) \leq k$.
	
	Conversely, we suppose that there exists \winstrategy be a winning 
	MD-strategy for \ReachPl such that 
	$\dhamm^s(\loosestrategy, \winstrategy) \leq k$ and we prove that all 
	vertices of $\loc \in C_{\ReachPl}$ are such that $\winstrategy(\loc) 
	\neq \loosestrategy(\loc)$. In particular, from all vertices 
	$\loc \notin C_{\ReachPl}$ such that $\winstrategy(\loc) \neq 
	\loosestrategy(\loc)$, then we can apply Lemma~\ref{lem:find-win_trans} 
	to define \strategy be a winning MD-strategy that is $C_{\ReachPl}$-distinct 
	\loosestrategy-strategy. Moreover, $\dhamm^s(\loosestrategy, \strategy) \leq 
	\dhamm^s(\loosestrategy, \winstrategy) \leq k$ (since we only synchronise 
	some choices of \strategy to \loosestrategy and by hypothesis).
	
	To conclude this proof, we prove that all vertices of $\loc \in C_{\ReachPl}$ 
	are such that $\winstrategy(\loc) \neq \loosestrategy(\loc)$. We reason by 
	contradiction and we suppose that there exists $\loc \in C_{\ReachPl}$ 
	are such that $\winstrategy(\loc) = \loosestrategy(\loc)$. In particular, 
	by definition of $C_{\ReachPl}$ given by~\eqref{eq:c-Reach}, 
	$\loosestrategy(\loc) \in \Trans \setminus \Trans^*_{\LocsT}$. We distinguish 
	two cases. First, we suppose that $\loosestrategy(\loc) = (\loc, \loc')$ 
	with $\loc' \notin \Locs^*_{\LocsT}$. Thus, \winstrategy is not winning from 
	\loc. To conclude, either $\loc \in \Locs^{\winstrategy}$ and \winstrategy is 
	not winning, or $\loc \notin \Locs^{\winstrategy}$ and we can define 
	$\winstrategy(\loc)$ such that $\winstrategy(\loc) \neq \loosestrategy(\loc)$.
	Finally, we suppose that $\loosestrategy(\loc) = (\loc, \loc')$ 
	with $\loc' \in \Locs^*_{\LocsT}$. To conclude, either $(\loc, \loc') \in 
	\Trans^*_{\LocsT}$ that is a contradiction, or $(\loc, \loc') \notin 
	\Trans^*_{\LocsT}$ and $\loc' \in \Locs^*_{\LocsT}$ there exists a 
	cycle around $\loc'$ that is a \winstrategy-play. Thus, \winstrategy is 
	non-winning.
	\qed
\end{proof}







==> sections/explain-game.tex <==
\section{Explanation of losing for \ReachPl}
\label{sec:explain_game}

Let $\game$ be a reachability game where \ReachPl loses, i.e. \ReachPl do not 
have any winning strategy. Our goal is to explain why a such strategy does not 
exists. In particular,  we do not use a non-winning strategy for \ReachPl. 
Unlike for other causes, we directly define a cause on the game without any 
restriction given by a non-winning strategy of \ReachPl. Intuitively, a 
game-cause defines a set of vertices that \ReachPl need to control to win the 
game. Formally, we define a game-cause for \game in the following definition.

\begin{definition}
	\label{def:game_game-cause}
	Let $C \subseteq \LocsSafe$ be a set of vertices of \SafePl. We said that 
	$C$ is a \emph{game-cause} if there exists a winning strategy for \ReachPl 
	in $\game_C = (\LocsReach \cup C, \LocsSafe \setminus C, \Trans)$, 
	i.e. there exists a winning strategy for \ReachPl when we change the 
	belong of vertices in $C$. \markend
\end{definition}

\begin{figure}[tbp] 
	\centering
	\begin{tikzpicture}[xscale=.7,every node/.style={font=\footnotesize}, 
	every label/.style={font=\scriptsize}]
	\node[PlayerReach] at (0,0) (s0) {$\loc_0$};
	\node[PlayerSafe] at (0,-2) (s1) {$\loc_1$};
	\node[PlayerSafe] at (3,0) (s2) {$\loc_2$};
	\node[PlayerReach] at (3,-2) (s3) {$\loc_3$};
	\node[PlayerSafe] at (6,2) (s4) {$\loc_4$};
	\node[PlayerReach] at (6,-2) (s5) {$\loc_5$};
	\node[target] at (6,0) (e) {$\LocsT$};
	
	\draw[->]
	(s0) edge[bend right=10] (s1)
	(s0) edge (s2)
	(s1) edge[bend right=10] (s0)
	(s1) edge (s3)
	(s2) edge (s1)
	(s2) edge (s4)
	(s2) edge (s5)
	(s2) edge (e)
	(s3) edge (s2)
	(s3) edge (s5)
	(s4) edge (e)
	(s5) edge (e)
	;
	\end{tikzpicture}
	\caption{A reachability games, with \locinit be an initial vertex, where 
		\ReachPl looses.}
	\label{fig:game_cause-1}
\end{figure}


\begin{example}
	\label{ex:game_game-cause}
	We consider the reachability game depicted in 
	\figurename{\ref{fig:game_cause-1}}. We fix $C = \{\loc_2\}$ be a 
	game-cause since $\winstrategy(\loc_0) = (\loc_0, \loc_2)$, and 
	$\winstrategy(\loc_2) = \LocsT$ define a winning strategy for \ReachPl. 
	\markend 
\end{example}

\paragraph{Checking a game-cause.} Unlike in transition-cause or state-cause, 
to check if a set of vertices of \SafePl is a game-cause, we can directly 
apply the definition, i.e. we simply check if \ReachPl wins the game when we 
change the belong of $C$. Thus, we can check in polynomial time in size of \game.

\begin{proposition}
	\label{prop:game_check-game}
	Let \game be a reachability game where \ReachPl loses, and a potential cause 
	$C \subseteq \LocsSafe$. We can check if $C$ is a game-cause in polynomial 
	time. 
\end{proposition}
\begin{proof}
	We define $\game_C$ be the reachability game given in 
	Definition~\ref{def:game_game-cause}, i.e.  
	$\game_C = (\Locs', \locinit, \Trans)$ such that 
	$\Locs' = (\LocsReach \cup C, \LocsSafe \setminus C, \LocsT)$. By 
	definition, $C$ is a game-cause if and only if \ReachPl wins in $\game_C$. 
	Since the size of \game and $\game_C$ are the same, testing if \ReachPl wins 
	in $\game_C$ is done in polynomial time in size of \game. \qed
\end{proof}

\subsection{Existence of a game-cause}
\label{subsec:game_existence}

The existence of a game-cause is not guaranteed in all reachability games. 
However, a game-cause exists when there exists a path from \locinit to \LocsT in 
the underlying graph of \game, i.e. in the one-player game over the graph of 
\game. In particular, a game-cause will be the whole set of vertices of \SafePl. 
Thus, test if \LocsSafe is a game-cause suffice to check if a such cause exists, 
and we can do it in polynomial time.

\begin{proposition}
	\label{prop:game_find-game}
	Let \game be a reachability game where \ReachPl loses. Testing the existence 
	of a game-cause can be done in polynomial time in size of \game. 
\end{proposition}

The proof of this proposition is given by the monotony of game-cause. Indeed, 
when \ReachPl controls a set of vertices of \SafePl to win, if we add some 
vertices, \ReachPl still wins whatever his strategy does in these new vertices. 
We note that transition-causes and state-causes are not monotones.

\begin{lemma}[Monotony]
	\label{lem:game_monotony}
	Let \game be a reachability game where \ReachPl looses and $C$ be a 
	game-cause. Let $C' \subseteq \LocsSafe$ such that $C \subseteq C'$, 
	then $C'$ is a game-cause.
\end{lemma}
\begin{proof}
	Let \winstrategy be the winning strategy in $\game_C = (\LocsReach \cup C, 
	\LocsSafe \setminus C, \Trans)$ (there exists since $C$ is a game-cause). 
	Now, we define \strategy be a strategy in $\game_{C'} = (\LocsReach \cup C', 
	\LocsSafe \setminus C', \Trans)$ such that 
	\begin{displaymath}
	\strategy(\loc) = 
	\begin{cases}
	\winstrategy(\loc) & \text{if $\loc \in \LocsReach \cup C$} \\ 
	(\loc, \loc') & \text{otherwise, with $(\loc, \loc') \in \Trans$}
	\end{cases}
	\end{displaymath}
	Since \winstrategy be the winning strategy in $\game_C$, all 
	\winstrategy-plays reach \LocsT. In particular, all \winstrategy-plays that 
	through by $\loc \in C' \setminus C$ reach \LocsT. Thus, \strategy is 
	winning.
	\qed
\end{proof}

Now, we have tools to prove Proposition~\ref{prop:game_find-game}.

\begin{proof}[Proof of Theorem~\ref{prop:game_find-game}]
	To conclude the proof, we need to prove that \LocsSafe is a game-cause if 
	and only if there exists a game-cause in \game. Indeed, by 
	Proposition~\ref{prop:game_check-game}, we can test in polynomial time 
	if \LocsSafe is a game-cause.
	
	Now, if \LocsSafe is a game-cause, then there exists a game-cause in \game. 
	Conversely, we suppose that there exists $C$ be a game-cause in \game. 
	In particular, by Lemma~\ref{lem:game_monotony}, since 
	$C \subseteq \SafePl$, \SafePl is a game-cause. 
	\qed
\end{proof}


\subsection{Finding a minimal-size game-cause}
\label{subsec:game_finding}
\todo[inline]{Might this not be NP-hard as well?
Proof idea: Reduction from feedback vertex set: Let $G=(V,E)$ be a strongly connected graph and $k$ a natural number. It is NP-hard to decide whether it is possible to remove $k$ vertices from $G$ such that the remaining graph is acyclic.
Now construct the following game: It has locations $V$ and additional locations $\locinit$ and $e$. The initial location is $\locinit$. The target for $\ReachPl$ is $\LocsT=\{e\}$.
From $\locinit$, there is a transition to every location in $V$. From $t\in V$, there is a transition to $e$ and a transition to each $s\in V$ with $(t,s)\in E$.
All locations are controlled by $\SafePl$, i.e., $\LocsSafe=V\cup\{\locinit\}$. 
Now, there is a game cause for the fact that $\ReachPl$ loses of size $k$ if and only if one can remove $k$ vertices from $G$ such that the remaining graph is acyclic. (Removing a vertex corresponds to changing the corresponding location to belong to $\ReachPl$ such that $\ReachPl$ can choose to go to $e$ from there. If no cycles in $G$ are remaining,  $\SafePl$ cannot avoid to go into a location that now belongs to $\ReachPl$.}


\todo[inline]{To review}

Proposition~\ref{prop:game_find-game} gives us the expectation of \ReachPl to 
win in \game. However, it says nothing about important vertices that \ReachPl 
needs control to win. So, to refine the explanation for \ReachPl in this 
context, we want to compute a ”good” game-cause, i.e. a game-cause with a 
minimal number of vertices. In the following, we compute a game-cause with 
minimal size in polynomial time.

\begin{theorem}
	\label{thm:game_good-game}
	Let \game be a reachability game where \ReachPl looses in \game. Then, 
	we can compute a game-cause with a minimal size in polynomial time.
\end{theorem}

To compute a game-cause with minimal size, we compute a strategy from a payoff 
defining by a fixpoint. In particular, we define $\mathcal{F}$ be a function 
from $\Locs$ to $\mathcal{P}_{\LocsSafe} \cup \bot$ such that $|\bot| = +\infty$ 
and for all vertices \loc we have 
\begin{displaymath}
\mathcal{F}(X)(\loc) = 
\begin{cases}
\emptyset & \text{if $\loc \in \LocsT$} \\
\bot & \text{if $\loc \notin \LocsT$ and $E(\loc) = \emptyset$} \\
\minsize_{(\loc, \loc') \in \Trans(\loc)} \mathcal{F}(X)(\loc') & 
\text{if $\loc \in \LocsReach$} \\
\minsize 
\begin{cases}
\bigcup_{(\loc, \loc') \in \Trans(\loc)} \mathcal{F}(X)(\loc') \\ 
\{\loc\} \cup \minsize_{(\loc, \loc') \in \Trans(\loc)} \mathcal{F}(X)(\loc')
\end{cases}
& \text{if $\loc \in \LocsSafe$} 
\end{cases}
\end{displaymath}
where \minsize is an operator over sets that gives the set with the minimum size. 
In particular, we note that for all set $S$, $\minsize(S, \bot) = S$ and 
$S \cup \bot = \bot$.
Intuitively, for all vertices $\mathcal{F}$ compute the minimum vertices that 
\ReachPl needs to control to win. Indeed, for all vertices of \SafePl, $\mathcal{F}$ 
chooses to between keep this vertex belongs to \SafePl or change his belong. 
In the case of $\mathcal{F}$ chooses to keep this vertex belongs to \SafePl, to 
wins \ReachPl needs to control all vertices of \SafePl needed from all its neighbour 
(i.e. we need to compute the union). Otherwise, since \ReachPl controls the vertex, 
he can chooses to restrict the set of plays by choosing only one edge and obtain 
control the minimal number of vertices from the vertex given by the edge. 

Now, we note by $\C$ the fixpoint of $\mathcal{F}$ obtain by value iteration 
of $\mathcal{F}$ from $\C^0$ such that $\C^0(\loc) = \bot$ when $\loc \notin \LocsT$, 
and $\C^0(\loc) = \emptyset$ otherwise. Then, for all $i > 0$, we fix 
$\C^i = \mathcal{F}^i(\C^0)(\loc)$ be the iteration $i$ of $\mathcal{F}$.
Intuitively, $\C^i(\loc)$ is the set of vertices of \SafePl with a minimal size that 
\ReachPl needs control to win from \loc within $i$ steps. 

\begin{lemma}
	\label{lem:game-find_1}
	Let \loc be a vertex of \game where \ReachPl looses. Then, $\C^i(\loc)$ is the 
	set of vertices of \SafePl with a minimal size such that \ReachPl wins within 
	$i$ steps from \loc in $\game_{\C^i}$ when it is possible, otherwise 
	$\C^i = \bot$. 
\end{lemma}
\begin{proof}
	We reason by induction on $i$ to prove that for all vertices $\loc \in \Locs$, 
	$\C^i(\loc)$ is the set of vertices of \SafePl with a minimal size such that 
	\ReachPl wins within $i$ steps from \loc in $\game_{\C^i}$ when it is possible, 
	otherwise $\C^i = \bot$.
	First, we suppose that $i = 0$. Since \ReachPl can wins in $0$ steps only 
	in vertices of \LocsT, then $\C^0$ satisfies the property. Now, we suppose 
	that the property holds for $i \geq 0$. Let $\loc \in \Locs$, and we suppose 
	that $\loc \in \LocsT$. In this case, $\C^{i+1}(\loc) = \emptyset$ and \ReachPl 
	can win within $0$ steps from \loc. Now, we suppose that 
	$\Trans(\loc) = \emptyset$ with $\loc \notin \LocsT$. In this case 
	$\C^{i+1}(\loc) = \bot$ and \ReachPl can not win (within $i+1$ steps) from \loc.  
	
	Now, we suppose that $\loc \in \LocsReach$ and by definition of $\mathcal{F}$, 
	$\C^{i+1}(\loc) = \C^i(\loc')$ where $\loc'$ is such that 
	$\C^i(\loc') = \minsize_{(\loc, \loc') \in \Trans(\loc)} 
	\mathcal{F}(\C^i)(\loc')$. If $\C^{i+1}(\loc)  = \bot$, then \ReachPl can 
	not win within $i+1$ steps from \loc, since for all $(\loc, \loc') \in E(\loc')$, 
	$\C^i(\loc') = \bot$ (by minimum) and \ReachPl can not win within $i$ steps 
	from $\loc'$ (by hypothesis of induction). Otherwise, $\C^{i+1}(\loc) \neq \bot$, 
	and by induction of hypothesis applied on $\loc'$, there exits a winning 
	memoryless strategy \winstrategy in $\game_{\C^i(\loc')}$ from $\loc'$. So, 
	let \strategy be a strategy in $\game_{\C^i(\loc')}$ such that for all vertices 
	$\loc''$, $\strategy(\loc'') = \winstrategy(\loc'')$ if $\loc'' \neq \loc$, and 
	$\strategy(\loc) = (\loc, \loc')$. Thus, since \winstrategy is winning from 
	$\loc'$ within $i$ steps, \strategy is winning from \loc within $i+1$ steps. 
	Moreover, by minimum over all possible neighbour of \loc, $\C^i(\loc')$ has 
	a minimum size, i.e. $\C^{i+1}(\loc)$ has a minimal size.
	
	Finally, we suppose that $\loc \in \LocsSafe$. If $\C^{i+1}(\loc) = \bot$ then, 
	for all neighbour $\loc'$ of \loc, $\C^{i}(\loc') = \bot$ (otherwise it suffices 
	to control \loc) and \ReachPl can not win within $i$ steps from $\loc'$ (by 
	hypothesis of induction). Otherwise $\C^{i+1}(\loc) \neq \bot$. First, we 
	suppose that $\C^{i+1}(\loc) = \bigcup_{(\loc, \loc') \in \Trans(\loc)} 
	\mathcal{F}(\C^i)(\loc')$, and we conclude that \ReachPl wins in 
	$\game_{\C^i(\loc)}$ from \loc within $i+1$ steps by applying hypothesis of 
	induction on all $\loc'$ (and by combining the winning strategies from each 
	$\loc'$: in the case where two wining strategies make distinct choices in same 
	vertex, then we simply take one of them since both are winning).
		\todo[inline]{Jakob: I do not see why $\C^{i+1}(\loc)$ is guaranteed to be minimal in this case.}

	
	Now, we suppose that $\C^{i+1}(\loc) = \{\loc\} \cup 
	\minsize_{(\loc, \loc') \in \Trans(\loc)} \mathcal{F}(\C^i)(\loc') = 
	\{\loc\} \cup \C^i(\loc')$. In this case, \ReachPl needs to control \loc. In 
	particular, by applying the hypothesis of induction on $\loc'$, we prove that 
	\ReachPl wins within $i+1$ steps in $\game_{\C^{i+1}(\loc)}$ with 
	$\winstrategy(\loc) = (\loc, \loc')$ and other by the strategy given by 
	hypothesis. To conclude, we remark that $\C^{i+1}(\loc)$ by definition of 
	$\mathcal{F}$.
\end{proof}


Since $\mathcal{F}$ is monotone and for each vertex there exists a lower bound (i.e. 
$\emptyset$), then value iteration of $\mathcal{F}$ converge to $\C$. Moreover,
this convergence is done in $|\Locs|$ iterations (since at each step a new 
vertices of \SafePl can be control by \ReachPl or the fixpoint is reached).

\begin{lemma}
	Let $\game = (\Locs, \locinit, \Trans)$ be a reachability game where \ReachPl 
	looses. Then, $\mathcal{F}^{|\Locs|}(\C^0) = \mathcal{F}^{|\Locs|+1}(\C^0)$. 
\end{lemma}
\begin{proof}
	We reason by contradiction and we suppose that there exists \loc such that 
	$\mathcal{F}^{|\Locs|}(\C^0)(\loc) > \mathcal{F}^{|\Locs|+1}(\C^0)(\loc)$ 
	(the other case is not possible by monotony of $\mathcal{F}$). By definition, 
	$E(\loc) \neq \emptyset$ and $\loc \notin \LocsT$. If $\loc \in \LocsReach$, 
	then by Lemma~\ref{lem:game-find_1}, \ReachPl wins in $\game_{\C^{|\Locs| + 1}}$ 
	within $|\Locs|+1$ steps by not in $|\Locs| + 1$. We have a contradiction since 
	\ReachPl wins without cycles.
	
	Otherwise, $\loc \in \LocsSafe$ and $\mathcal{F}^{|\Locs|}(\C^0)(\loc) \neq \bot$ 
	(otherwise contradiction since \ReachPl wins without cycles). Moreover, by 
	Lemma~\ref{lem:game-find_1}, \ReachPl wins in $\game_{\C^{|\Locs| + 1}}$ 
	within $|\Locs|+1$ steps by not in $|\Locs| + 1$ (since wins without cycle).
\end{proof}



==> sections/games.tex <==
\section{Causality in reachability games}
\todo[inline]{Rename, merge with next section, and clean-up}


We want to define counterfactual causes for reachability games to explain
for Player $i$ 
\begin{enumerate}
	\item\label{item:game_task1} why a strategy is non-winning whether Player 
	$i$ wins the game; 
	\item\label{item:game_task2} why Player $i$ loses the game.
\end{enumerate} 
This explanation can be a set of vertices to avoid (like in a transition 
system), or a set of forbidden edges, or again a set of vertices of that 
Player $i$ must control to win the game, i.e. we can define three types of 
causes.

Now, we consider a two-player turn-based reachability game 
$\game = (\Locs, \Trans, \LocsT)$ with a \ReachPl player (i.e. Player $0$) 
that wants to reach the effect and a \SafePl player (i.e. Player $1$) that 
never wants to reach it. Now, if Player $i$ loses the game, we want to 
explain why he can not win. Otherwise, we consider a (memoryless) non-winning 
strategy \loosestrategy for Player $i$, and we want to explain what is wrong 
with this strategy. In this case, we have two ways to explain it according to 
the presence of \loosestrategy-play in the specification of the problem. 
Thus, we can define three problems:
\begin{description}
	\item[Counterfactual explaination] "What goes wrong with \loosestrategy 
	according to \looseplay ?" where \looseplay is a non-winning 
	\loosestrategy-play. 
	
	\item[Explaination of non-winning] "What goes wrong with \loosestrategy 
	?" when Player $i$ wins in \game;

	\item[Explaination of losing] "Why is there is no winning strategy ?" 
	when Player $i$ loses in \game.
\end{description}
In this work, we will focus on the \emph{counterfactual explanation} for 
\SafePl player that is a really closed problem to counterfactual cause in 
transition systems. Then, we will focus on the \emph{explanation of 
non-winning} (Section~\ref{sec:explain-strat}) and on the 
\emph{explanation of losing} (Section~\ref{sec:explain_game}) for \ReachPl 
player.


\paragraph{Results on causality in games.} 
In Sections~\ref{sec:explain-strat} and~\ref{sec:explain_game}, we study the 
explanation of non-winning and of losing with three problems: the checking 
problem that consists of the test of a candidate cause, the existence problem 
that tests if there exists a cause for a reachability game (and a non-winning 
strategy), and the finding a ”good” cause according to some criterion of 
quality (like distances between two memoryless strategies). 
Table~\ref{table:game_results}  summarizes our results.

\begin{table}[tbp]
	\centering
	\begin{tabular}{c|c|c|c|c|c|}
		\multirow{2}{*}{Causes} & \multirow{2}{*}{Checking} & 
		\multirow{2}{*}{Existence} &  
		\multicolumn{3}{|c|}{Finding a "good" cause} \\
		\cline{4-6}
		& &  & Size & Hamming & Hausdorff-Hamming \\
		\hline
		Transition & 
		\multirow{4}{1.5cm}{\centering in P (Prop.~\ref{prop:game_check})} & 
		\multirow{4}{1.5cm}{\centering in P (Thm.~\ref{thm:game_find})} & 
		NP-complete & NP-complete & NP-complete 
		(Thm.~\ref{thm:transition_finding-NP-c})  \\
		(Def.~\ref{def:game_transition-cause}) & & & 
		(Cor.~\ref{cor:fiding-trans_minsize}) & 
		(Thm.~\ref{thm:transition_finding-NP-c}) & in P for acyclic 
		$\game^{\loosestrategy}$ (Thm.~\ref{thm:find-trans_poly}) \\
		\cline{1-1}
		\cline{4-6}
		State & & & \multicolumn{3}{|c|}{NP-complete}  \\
		(Def.~\ref{def:game_state-cause}) & & & 
		\multicolumn{3}{|c|}{(Cor.~\ref{cor:fiding-loc})} \\
		\hline
		Game & in P & in P & in P & 
		\multicolumn{2}{|c|}{\multirow{2}{*}{Not relevant}}  \\ 	
		(Def.~\ref{def:game_game-cause}) & (Prop.~\ref{prop:game_check-game}) & 
		(Prop.~\ref{prop:game_find-game}) & (Thm.~\ref{thm:game_good-game}) 
		& \multicolumn{2}{|c|}{}	\\	
		\hline
	\end{tabular}
	\caption{Contribution on causality in games.}
	\label{table:game_results}
\end{table}

\subsubsection{Some distances for memoryless strategies}
\label{subsubsec:games_distance}

\todo[inline]{Its position? - To review...}

In the context of game, we do not use (for instance) distance to define the 
notion of cause. However, we define some distance over memoryless strategies to 
obtain a quality criterion for a transition-cause. A "good" transition-cause 
exhibits a winning strategy that minimises its distance to the non-winning 
strategy. 

In this Section, we look to answer the question "How define a distance between 
two memoryless strategies?". Unless in the case of transitions systems, here we 
want to compare a set of plays. To do that, we will use an usual distance for 
topology theory: the Hausdorff 
distance\footnote{\url{https://en.wikipedia.org/wiki/Hausdorff_distance}}. 

\begin{definition}
	Let \winstrategy and \loosestrategy be two memoryless strategy, and 
	$\dist$ be a distance over plays (see like a string, or a path in a TS). 
	The Hausdorff distance of this two strategies is defined by 
	\begin{displaymath}
	\dhaus{\dist}(\loosestrategy, \winstrategy) = 
	\max \left\{ \sup_{\substack{$\looseplay$ \\ \text{$\loosestrategy$-play}}} 
	\inf_{\substack{$\winplay$ \\ \text{$\winstrategy$-play}}} 
	\dist(\looseplay, \winplay),  
	\sup_{\substack{\winplay \\ \text{\winstrategy-play}}} 
	\inf_{\substack{\looseplay \\ \text{\loosestrategy-play}}} 
	\dist(\looseplay, \winplay) \right\}
	\end{displaymath}
\end{definition} 


\todo[inline]{Jakob: Thoughts on the Hausdorff-prefix distance $\dpref^H$ (Hausdorff metric induced by the prefix metric):
For two strategies $\sigma$ and $\tau$, the distance $\dpref^H(\sigma,\tau)$ can be determined in terms of the $n$-round unfolding of the strategies as trees of possible $n$-round plays according to the strategy. We can increase $n$ until we reach a $N$ such that the $N$-round unfoldings of the two strategies are not identical anymore. Then, $\dpref^H(\sigma,\tau)=2^{-N}$.}
\todo[inline]{Jakob: Maybe, checking counterfactual causality can then be done by an iterative ATL (alternating-time temporal logic) model checking algorithm as the CTL algorithm for $\dpref$ in transition systems.
(In fact, this probably does not require ATL, but just solving a several reachability games)}

We note that we can instantiate this distance with all distances over string 
that we want. In particular with the prefix distance or the Hamming distance.


So, in this work, we will consider two distances based on the concept of the 
Hamming distance: 
\begin{enumerate}
	\item A Hausdorff-Hamming distance: that is the Hausdorff distance applying 
	to the Hamming distance; 
	
	\item A Hamming distance for games (a natural definition for memoryless 
	strategies): 
	\begin{equation}
	\label{eq:dHamm}
	\dhamm(\winstrategy, \loosestrategy) = 
	|\{\loc \in \Locs ~|~ \winstrategy(\loc) \neq \loosestrategy(\loc) \}|
	\end{equation}
\end{enumerate}

\paragraph{The Hausdorff-Hamming distance.} 
Intuitively, the Hausdorff-Hamming distance computes the maximal between the 
difference in choices along \loosestrategy-play regarding \winstrategy, and the 
difference in choices along \winstrategy-play regarding \loosestrategy. In 
particular, before to define this distance, we will define a distance between 
a play and a memoryless strategy.

Formally, let \loosestrategy be a memoryless strategy, and 
$\winplay = (\loc_0, \dots, \loc_n, \dots)$ be a play (not necessary a 
\loosestrategy-play or finite). The \emph{distance between \loosestrategy and 
	\winplay}, denoted by $\dist(\winplay, \loosestrategy)$, is the number of 
vertices of \winplay that are no conforming to \loosestrategy, i.e. it is the 
number of vertex $\loc \in \LocsReach$ such that there exists $i \in \N$ such 
that $\loc = \loc_i$ in \winplay, and $\loosestrategy(\loc_i) \neq 
(\loc_i, \loc_{i+1})$.


\begin{example}
	\label{ex:distance_strat-play}
	We consider the reachability game \game depicted in 
	\figurename{\ref{fig:ex_dHH}}, with the winning strategy \winstrategy 
	depicted in green. Let $\winplay = (\loc_0, (\loc_1, \loc_2, 
	\loc_3)^{\omega})$ be a play on \game (that is conforming with the 
	non-winning strategy \loosestrategy). On \winplay, we see that the choice is 
	distinct to \winstrategy in vertices $\loc_1$ and $\loc_3$. Thus, 
	$\dist(\winplay, \loosestrategy) = 2$.  
	\markend
\end{example}

\begin{remark}
	Be careful, $\dist(\winplay, \loosestrategy)$ does not give the number of 
	occurrences of vertices where \winplay is not conforming to \loosestrategy, 
	but the number of vertices. In particular, $\dist(\winplay, \loosestrategy)$ 
	is always finite even if \winplay is infinite. However, if we change to 
	compute the number of occurrence, the distance can become $+\infty$: we 
	consider the same strategy and play than in 
	Example~\ref{ex:distance_strat-play}, and since \winplay is not a finite play, 
	the number of occurrences of $\loc_1$ (or $\loc_3$) is $+\infty$. Thus, under 
	this definition, we can not deal with problem of the classical 
	Hausdorff-Hamming distance.
	\markend
\end{remark}

Now, we can define the Hausdorff-Hamming distance.

\begin{definition}
	Let \loosestrategy and \winstrategy be two memoryless strategy in the same 
	reachability game \game. The \emph{Hausdorff-Hamming distance} between 
	\loosestrategy and \winstrategy, denoted by $\dHH(\winstrategy, 
	\loosestrategy)$, is defined such that 
	\begin{displaymath}
	\dHH(\winstrategy, \loosestrategy) = 
	\max\left(\sup_{\substack{\winplay \\ \text{\winstrategy-play}}} 
	\dist(\winplay, \loosestrategy), 
	\sup_{\substack{\looseplay \\ \text{\loosestrategy-play}}} 
	\dist(\looseplay, \winstrategy)\right).
	\end{displaymath}
	\markend
\end{definition}

To simplify the notation, we denote by
\begin{displaymath}
\dstrat{\winstrategy}(\loosestrategy) = 
\sup_{\substack{\winplay \\ \text{\winstrategy-play}}} 
\dist(\winplay, \loosestrategy).
\end{displaymath}
Intuitively, for all memoryless strategies \winstrategy and \loosestrategy, 
$\dstrat{\winstrategy}(\loosestrategy)$ computes the similarity between 
\winstrategy-plays and \loosestrategy, i.e. how much \loosestrategy is closed 
to \winstrategy.

We start by given some properties on \dHH. In particular, we give some examples to 
illustrate the fact that there exists memoryless strategies \winstrategy and 
\loosestrategy such that $\dstrat{\loosestrategy}(\winstrategy) \neq 
\dstrat{\winstrategy}(\loosestrategy)$ (even if we make some minimality condition 
over \winstrategy), i.e.
\begin{enumerate}
	\item $\dist(\winplay, \loosestrategy) < \dist(\looseplay, \winstrategy)$ 
	(see Example~\ref{ex:dHH_looseplay});
	\item $\dist(\winplay, \loosestrategy) > \dist(\looseplay, \winstrategy)$ 
	(see Example~\ref{ex:dHH_winplay}).
\end{enumerate}

\begin{example}
	\label{ex:dHH_looseplay}
	We consider the game \game on the left of Figure~\ref{fig:ex_dHH} and the 
	non-winning strategy \loosestrategy depicted in green in the Figure. Now, 
	we consider \winstrategy, depicted in pink, be a winning and minimal 
	strategy for $\dstrat{\winstrategy}(\loosestrategy)$ (but not for $\dHH$) for 
	\ReachPl player. Now, we have for the first component: 
	\begin{displaymath}
	\dstrat{\winstrategy}(\loosestrategy)  
	= \max(\dist(\loc_0 ~ \loc_1 ~ \LocsT, \loosestrategy), 
	\dist(\loc_0 ~ \loc_3 ~ \LocsT, \loosestrategy)) = 1 
	\end{displaymath}
	and, for the second component, we have 
	\begin{displaymath}
	\dstrat{\loosestrategy}(\winstrategy) = 
	\dist((\loc_1 ~ \loc_2 ~ \loc_3)^{\omega}, \loosestrategy) = 2.
	\end{displaymath}
	
	We note that this \winstrategy, depicted in pink, is not minimal for 
	$\dHH$. Indeed, by the previous calculus, we have 
	$\dHH(\winstrategy, \loosestrategy) = 2$. Now, we consider \strategy a 
	winning strategy for \ReachPl such that $\strategy(\loc_1) = 
	\loosestrategy(\loc_1)$ and $\strategy(\loc_3) = \winstrategy(\loc_3)$. In 
	this case, we have for the first component: 
	\begin{displaymath}
	\dstrat{\winstrategy}(\loosestrategy) 
	= \max(\dist(\loc_0 ~ \loc_1 ~ \loc_2 ~ \loc_3 ~ \LocsT, \loosestrategy), 
	\dist(\loc_0 ~ \loc_3 ~ \LocsT, \loosestrategy)) = 1 
	\end{displaymath}
	and, for the second component, we have 
	\begin{displaymath}
	\dstrat{\loosestrategy}(\winstrategy) = 
	\dist((\loc_1 ~ \loc_2 ~ \loc_3)^{\omega}, \loosestrategy) = 1.
	\end{displaymath}
	Thus, $\dHH(\strategy, \loosestrategy) = 2$ that is optimal by  
	Lemma~\ref{lem:dHH_bound}.
	\markend
\end{example}

Moreover, the previous example show that there exists a winning strategy 
\winstrategy for \ReachPl player minimal for 
$\dstrat{\winstrategy}(\loosestrategy)$, but not for  
$\dstrat{\loosestrategy}(\winstrategy)$. However, it is not a counter-example for 
the existence of a strategy that minimize (over winning strategy) both 
component of the distance $\dHH$.

\begin{example}
	\label{ex:dHH_winplay}
	We consider the game \game on the right of Figure~\ref{fig:ex_dHH} and the 
	non-winning strategy \winstrategy depicted in green in the Figure. Now, 
	we consider \winstrategy, depicted in pink, be a winning and minimal 
	strategy for $\dHH$ for \ReachPl player (since it is the only other one). 
	Now, we have only one \winstrategy-play 
	$\winplay = \loc_1 \to \loc_3 \to \LocsT$, and one \loosestrategy-play 
	$\looseplay = \loc_1 \to \loc_2^{\omega}$. Thus,
	\begin{displaymath}
	\sup_{\substack{\winplay \\ \text{\winstrategy-play}}} 
	\dist(\winplay, \loosestrategy) = 2 
	\qquad \text{and} \qquad
	\sup_{\substack{\looseplay \\ \text{\loosestrategy-play}}} 
	\dist(\looseplay, \winstrategy) = 1.
	\end{displaymath}
	Thus, we deduce that we have $\dHH(\winstrategy, \loosestrategy) = 2$ (that 
	is optimal since \winstrategy is the only winning strategy). 
	\markend
\end{example}

To conclude this, part we will show that for all winning strategy \winstrategy, 
we have $\dHH(\winstrategy, \loosestrategy) \in [1, |\game|]$.

\begin{lemma}
	\label{lem:dHH_bound}
	Let \game be a reachability game, \loosestrategy be a non-winning 
	strategy for \ReachPl, and \winstrategy ba a winning strategy for 
	\ReachPl. We have $1 \leq \dHH(\winstrategy, \loosestrategy) \leq 
	|\LocsReach|$.
\end{lemma}
\begin{proof}
	By definition of $\dist$, $\dHH(\winstrategy, \loosestrategy) \leq 
	|\LocsReach|$, since we compute the number of vertices of \ReachPl such 
	that the choice is not conforming to a memoryless strategy.
	
	Now, since \winstrategy is a winning strategy for \ReachPl and 
	\loosestrategy is a non-winning strategy, we know that there exists 
	a \winstrategy-play \winplay such that \winplay is not a 
	\loosestrategy-play (otherwise \winstrategy is not a winning strategy), 
	and $1 \leq \dist(\winplay, \loosestrategy) \leq 
	\dstrat{\winstrategy}(\loosestrategy) \leq 
	\dHH(\loosestrategy, \winstrategy)$.
	\qed
\end{proof}

\paragraph{The Hamming distance}
In parallel of the Hausdorff-Hamming distance, we can define the Hamming 
distance (by~\eqref{eq:dHamm}) for memoryless strategies to compute the 
number of choices that are distinct between two memoryless strategies. 
Like for the Hausdorff-Hamming distance, we can bound the Hamming distance 
for all winning strategy against a non-winning strategy.

\begin{lemma}
	\label{lem:dHamm_bound}
	Let \game be a reachability game, \loosestrategy be a non-winning 
	strategy for \ReachPl, and \winstrategy ba a winning strategy for 
	\ReachPl. We have $1 \leq \dhamm(\winstrategy, \loosestrategy) \leq 
	|\LocsReach|$.
\end{lemma}
\begin{proof}
	By definition, we compute the number of vertices of \ReachPl such 
	that the choice is not conforming to a memoryless strategy, so 
	$\dhamm(\winstrategy, \loosestrategy) \leq 
	|\LocsReach|$
	
	Now, since \winstrategy is a winning strategy for \ReachPl and 
	\loosestrategy is a non-winning strategy, we know that there exists 
	a vertex \loc in \game such that $\winstrategy(\loc) \neq 
	\loosestrategy(\loc)$. Otherwise, both strategies are equal and a strategy 
	can not be a winning and a non-winning strategy. Thus,
	$1 \leq \dhamm(\loosestrategy, \winstrategy)$.
	\qed
\end{proof}

The Hamming distance is not comparable with the Hausdorff-Hamming distance. 
Intuitively, the Hausdorff-Hamming distance give only the number of choices 
that are distinct between two memoryless strategies according the choices of 
\SafePl player. Thus, the two distance may be distinct, and a strategy that 
minimise the Hausdorff-Hamming distance may not minimise the Hamming distance
(see Example~\ref{ex:dHamm}). The converse seems to be true. \todo{To prove it?}

\begin{figure}[tbp]
	\centering
	\begin{tikzpicture}[xscale=.7,every node/.style={font=\footnotesize}, 
	every label/.style={font=\scriptsize}]
	\node[PlayerReach] at (0, 0) (v0) {$\loc_0$};
	\node[PlayerSafe] at (3, 0) (v1) {$\loc_1$};
	\node[PlayerReach] at (6, -1) (v2) {$\loc_2$};
	\node[PlayerReach] at (6, 1) (v3) {$\loc_3$};
	\node[target] at (-3, 0) (t1) {$\LocsT$};
	\node[target] at (9, 0) (t2) {$\LocsT$};
	\node[target] at (9, -1) (t3) {$\neg \LocsT$};
	\node[target] at (9, 1) (t4) {$\neg \LocsT$};
	
	\node[strat] at (2,0) (st) {};
	\node[strat] at (8,-1) (st11) {};
	\node[strat] at (8, 1) (st12) {};
	\node[strat] at (7.5,-.5) (st21) {};
	\node[strat] at (7.5,.5) (st22) {};
	
	% Connect the states with arrows
	\draw[->] 
	(v0) edge (v1)
	(v0) edge (t1)
	(v1) edge (v2)
	(v1) edge (v3)
	(v2) edge (t2)
	(v2) edge (t3)
	(v3) edge (t2)
	(v3) edge (t4)
	
	(v0) edge[RoyalBlue, line width=0.5mm] node[above] 
	{\textcolor{RoyalBlue}{\winstrategy,\loosestrategy}} (st)
	(v2) edge[ForestGreen, line width=0.5mm] node[below] 
	{\textcolor{ForestGreen}{\loosestrategy}} (st11)
	(v3) edge[ForestGreen, line width=0.5mm] node[left,yshift=.1cm] 
	{\textcolor{ForestGreen}{\loosestrategy}} (st12)
	(v2) edge[Magenta, line width=0.5mm] node[left] 
	{\textcolor{Magenta}{\winstrategy}} (st21)
	(v3) edge[Magenta, line width=0.5mm] node[below,yshift=-.1cm] 
	{\textcolor{Magenta}{\winstrategy}} (st22);
	\end{tikzpicture}
	\caption{A reachability game where \winstrategy that minimises \dHH but 
		not $\dhamm$.}
	\label{fig:ex_dHamming}
\end{figure}

\begin{example}
	\label{ex:dHamm}
	We consider the reachability game \game depicted in 
	\figurename{\ref{fig:ex_dHamming}}, and the non-winning strategy 
	\loosestrategy depicted in green. The winning strategy \winstrategy depicted 
	in pink minimise the Hausdorff-Hamming distance, since for all 
	\winstrategy-plays, their distance to \loosestrategy is $1$, and for all 
	\loosestrategy-plays, their distance to \winstrategy is $1$ too. But, 
	\winstrategy do not minimise the Hamming distance, since 
	$\dhamm(\winstrategy, \loosestrategy) = 2$. Let consider \winstrategy' 
	be the winning strategy defined like \loosestrategy in $\loc_2$ and $\loc_3$, 
	but in $\loc_0$ chooses to go to \LocsT. For this strategy, 
	$\dhamm(\winstrategy, \loosestrategy) = 1$, and it is minimum. We note that 
	\winstrategy' minimise also the Hausdorff-Hamming distance.
\end{example}


The Hamming distance is an interesting distance since a winning strategy that 
minimise this distance defines a minimal size transition-cause.

\begin{lemma}
	\label{lem:hamm-size}
	Let \game be a reachability game, \loosestrategy be a non-winning strategy, 
	\winstrategy be a winning strategy such that it minimises the Hamming distance 
	with \loosestrategy, i.e. $\winstrategy = \min_{\strategy-\text{winning}} 
	\dhamm(\strategy, \loosestrategy)$. Then, the transition-cause given by 
	\winstrategy, $C^{\winstrategy}$, is a minimal size transition-cause.
\end{lemma}
\begin{proof}
	We reason by contradiction and we suppose that there exits $C$ be a 
	transition-cause such that $|C| < |C^{\winstrategy}|$. In particular, there 
	exits a winning strategy \strategy such that, for all vertices $\loc \in 
	\LocsReach$, $\strategy(\loc) \neq \loosestrategy(\loc)$ if and only if 
	$\loosestrategy(\loc) \in C$ (by Definition~\ref{def:game_transition-cause}). 
	We deduce, by definition of Hamming distance given by 
	Equation~\eqref{eq:dHamm}, that 
	\begin{displaymath}
	\dhamm(\loosestrategy, \strategy) = |C| \underbrace{<}_{\text{by hypothesis}} 
	|C^{\winstrategy}| = \dhamm(\loosestrategy, \winstrategy)
	\end{displaymath}. 
	Thus, we obtain a contradiction.
	\qed
\end{proof}




